Ordered Risk Minimization: Learning More from Less Data

We consider the worst-case expectation of a permutation invariant ambiguity set of discrete distributions as a proxy-cost for data-driven expected risk minimization. For this framework, we coin the term ordered risk minimization to highlight how results from order statistics inspired the proxy-cost. Specifically, we show how such costs serve as point-wise high-confidence upper bounds of the expected risk. The confidence level can be determined tightly for any sample size. Conversely we also illustrate how to calibrate the size of the ambiguity set such that the high-confidence upper bound has some user specified confidence. This calibration procedure notably supports $\phi$-divergence based ambiguity sets. Numerical experiments then illustrate how the resulting scheme both generalizes better and is less sensitive to tuning parameters compared to the empirical risk minimization approach.

==> assets/sandbox/boxes.tex <==
\begin{tikzpicture}

    \definecolor{brown1926061}{RGB}{192,60,61}
    \definecolor{darkgray176}{RGB}{176,176,176}
    \definecolor{darkslategray61}{RGB}{61,61,61}
    \definecolor{peru22412844}{RGB}{224,128,44}
    \definecolor{seagreen5814558}{RGB}{58,145,58}
    \definecolor{steelblue49115161}{RGB}{49,115,161}
    
    \begin{groupplot}[
        group style={group size=2 by 1},
        numeric axis,
        width=0.5\columnwidth,
        height=0.5\columnwidth,
        xtick={0,1,2,3},
        xticklabels={SAA,KL,TV,CVAR},
        xmin=-0.5, xmax=3.5,
        xticklabel style={rotate=90},
        tick label style={font=\footnotesize},
    ]
    \nextgroupplot[
        ymin=230, ymax=240,
    ]
    \path [draw=darkslategray61, fill=steelblue49115161, semithick]
    (axis cs:-0.4,231.550197120447)
    --(axis cs:0.4,231.550197120447)
    --(axis cs:0.4,234.191226896709)
    --(axis cs:-0.4,234.191226896709)
    --(axis cs:-0.4,231.550197120447)
    --cycle;
    \path [draw=darkslategray61, fill=peru22412844, semithick]
    (axis cs:0.6,232.514582746267)
    --(axis cs:1.4,232.514582746267)
    --(axis cs:1.4,233.895616629797)
    --(axis cs:0.6,233.895616629797)
    --(axis cs:0.6,232.514582746267)
    --cycle;
    \path [draw=darkslategray61, fill=seagreen5814558, semithick]
    (axis cs:1.6,231.513291733636)
    --(axis cs:2.4,231.513291733636)
    --(axis cs:2.4,233.89561610775)
    --(axis cs:1.6,233.89561610775)
    --(axis cs:1.6,231.513291733636)
    --cycle;
    \path [draw=darkslategray61, fill=brown1926061, semithick]
    (axis cs:2.6,231.513291730288)
    --(axis cs:3.4,231.513291730288)
    --(axis cs:3.4,233.89561610782)
    --(axis cs:2.6,233.89561610782)
    --(axis cs:2.6,231.513291730288)
    --cycle;
    \addplot [semithick, darkslategray61]
    table {%
    0 231.550197120447
    0 230.922653028514
    };
    \addplot [semithick, darkslategray61]
    table {%
    0 234.191226896709
    0 236.628514347995
    };
    \addplot [semithick, darkslategray61]
    table {%
    -0.2 230.922653028514
    0.2 230.922653028514
    };
    \addplot [semithick, darkslategray61]
    table {%
    -0.2 236.628514347995
    0.2 236.628514347995
    };
    \addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
    table {%
    0 309.27480996047
    0 247.239662186754
    0 272.054556457494
    0 241.956296049462
    0 251.597605495105
    0 247.192043511445
    0 244.233368416658
    0 252.86600364674
    0 294.508720637123
    0 239.699528761407
    0 282.95835734537
    0 240.866292335017
    0 260.153936686469
    0 241.159137730683
    0 254.503548424132
    0 349.428745382197
    0 238.706990281232
    0 342.008656823814
    0 241.989558789093
    0 375.043430031865
    0 279.95704605889
    0 285.303883946213
    0 241.311335337042
    0 256.120889572637
    0 332.920304106216
    0 283.860290535548
    0 248.038686798161
    0 428.193625997454
    0 350.00539634576
    0 257.775349963224
    0 279.026151784935
    0 286.705272187652
    0 320.624346361995
    0 269.888760341798
    0 310.741096286397
    0 265.717927708245
    0 240.576552136251
    0 241.186957057808
    0 239.976526233234
    0 311.911146978049
    0 240.879249166674
    0 252.233515335486
    };
    \addplot [semithick, darkslategray61]
    table {%
    1 232.514582746267
    1 230.930341261761
    };
    \addplot [semithick, darkslategray61]
    table {%
    1 233.895616629797
    1 235.934460789289
    };
    \addplot [semithick, darkslategray61]
    table {%
    0.8 230.930341261761
    1.2 230.930341261761
    };
    \addplot [semithick, darkslategray61]
    table {%
    0.8 235.934460789289
    1.2 235.934460789289
    };
    \addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
    table {%
    1 236.468204369368
    1 236.282442484147
    1 236.5232542056
    1 241.019801966879
    1 236.844590076523
    1 237.365715769178
    };
    \addplot [semithick, darkslategray61]
    table {%
    2 231.513291733636
    2 230.922503076188
    };
    \addplot [semithick, darkslategray61]
    table {%
    2 233.89561610775
    2 233.895616125469
    };
    \addplot [semithick, darkslategray61]
    table {%
    1.8 230.922503076188
    2.2 230.922503076188
    };
    \addplot [semithick, darkslategray61]
    table {%
    1.8 233.895616125469
    2.2 233.895616125469
    };
    \addplot [semithick, darkslategray61]
    table {%
    3 231.513291730288
    3 230.922503076182
    };
    \addplot [semithick, darkslategray61]
    table {%
    3 233.89561610782
    3 233.895616121114
    };
    \addplot [semithick, darkslategray61]
    table {%
    2.8 230.922503076182
    3.2 230.922503076182
    };
    \addplot [semithick, darkslategray61]
    table {%
    2.8 233.895616121114
    3.2 233.895616121114
    };
    \addplot [semithick, black]
    table {%
    -0.5 230.922482721782
    3.5 230.922482721782
    };
    \addplot [semithick, red]
    table {%
    -0.5 233.895616107733
    3.5 233.895616107733
    };
    \addplot [semithick, darkslategray61]
    table {%
    -0.4 232.632500440114
    0.4 232.632500440114
    };
    \addplot [semithick, darkslategray61]
    table {%
    0.6 233.596504457635
    1.4 233.596504457635
    };
    \addplot [semithick, darkslategray61]
    table {%
    1.6 233.884876617215
    2.4 233.884876617215
    };
    \addplot [semithick, darkslategray61]
    table {%
    2.6 233.884876618234
    3.4 233.884876618234
    };
    
    \nextgroupplot[
        ymin=-60, ymax=30,
    ]
    \path [draw=darkslategray61, fill=steelblue49115161, semithick]
    (axis cs:-0.4,-25.6890308114622)
    --(axis cs:0.4,-25.6890308114622)
    --(axis cs:0.4,-1.45048896012033)
    --(axis cs:-0.4,-1.45048896012033)
    --(axis cs:-0.4,-25.6890308114622)
    --cycle;
    \path [draw=darkslategray61, fill=peru22412844, semithick]
    (axis cs:0.6,13.0663726881325)
    --(axis cs:1.4,13.0663726881325)
    --(axis cs:1.4,21.6590523033854)
    --(axis cs:0.6,21.6590523033854)
    --(axis cs:0.6,13.0663726881325)
    --cycle;
    \path [draw=darkslategray61, fill=seagreen5814558, semithick]
    (axis cs:1.6,14.4910449726339)
    --(axis cs:2.4,14.4910449726339)
    --(axis cs:2.4,24.2024290131935)
    --(axis cs:1.6,24.2024290131935)
    --(axis cs:1.6,14.4910449726339)
    --cycle;
    \path [draw=darkslategray61, fill=brown1926061, semithick]
    (axis cs:2.6,15.6543825861303)
    --(axis cs:3.4,15.6543825861303)
    --(axis cs:3.4,24.9936781479305)
    --(axis cs:2.6,24.9936781479305)
    --(axis cs:2.6,15.6543825861303)
    --cycle;
    \addplot [semithick, darkslategray61]
    table {%
    0 -25.6890308114622
    0 -58.347480844538
    };
    \addplot [semithick, darkslategray61]
    table {%
    0 -1.45048896012033
    0 18.4005333648362
    };
    \addplot [semithick, darkslategray61]
    table {%
    -0.2 -58.347480844538
    0.2 -58.347480844538
    };
    \addplot [semithick, darkslategray61]
    table {%
    -0.2 18.4005333648362
    0.2 18.4005333648362
    };
    \addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
    table {%
    0 -102.757610901079
    0 -71.3284813868621
    0 -76.1319872188375
    0 -196.488409076203
    0 -148.785854928501
    0 -174.89721207012
    0 -73.6855960407518
    0 -127.680676068894
    0 -81.3313453018287
    0 -249.243126843006
    0 -170.1697672745
    0 -66.2772007807008
    0 -99.9473506213679
    0 -166.24896593697
    0 -72.7900241581331
    0 -111.037617215037
    0 -111.115481470117
    };
    \addplot [semithick, darkslategray61]
    table {%
    1 13.0663726881325
    1 1.00876390880111
    };
    \addplot [semithick, darkslategray61]
    table {%
    1 21.6590523033854
    1 28.2427710251418
    };
    \addplot [semithick, darkslategray61]
    table {%
    0.8 1.00876390880111
    1.2 1.00876390880111
    };
    \addplot [semithick, darkslategray61]
    table {%
    0.8 28.2427710251418
    1.2 28.2427710251418
    };
    \addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
    table {%
    1 -12.2298209716486
    1 -7.02612768771002
    1 -10.914276710663
    1 -2.96599017393112
    1 -9.01930981768081
    };
    \addplot [semithick, darkslategray61]
    table {%
    2 14.4910449726339
    2 0.337087428241631
    };
    \addplot [semithick, darkslategray61]
    table {%
    2 24.2024290131935
    2 28.5215051020295
    };
    \addplot [semithick, darkslategray61]
    table {%
    1.8 0.337087428241631
    2.2 0.337087428241631
    };
    \addplot [semithick, darkslategray61]
    table {%
    1.8 28.5215051020295
    2.2 28.5215051020295
    };
    \addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
    table {%
    2 -1.22791451928057
    2 -19.8360947817637
    2 -1.30310912532676
    2 -14.0482167319997
    2 -18.8023431435918
    2 -3.21427921188493
    2 -16.6410930116488
    };
    \addplot [semithick, darkslategray61]
    table {%
    3 15.6543825861303
    3 2.20596381880588
    };
    \addplot [semithick, darkslategray61]
    table {%
    3 24.9936781479305
    3 28.819354160853
    };
    \addplot [semithick, darkslategray61]
    table {%
    2.8 2.20596381880588
    3.2 2.20596381880588
    };
    \addplot [semithick, darkslategray61]
    table {%
    2.8 28.819354160853
    3.2 28.819354160853
    };
    \addplot [black, mark=diamond*, mark size=2.5, mark options={solid,fill=darkslategray61}, only marks]
    table {%
    3 -0.467573940775821
    3 -19.9357523971958
    3 1.24172475214672
    3 -0.328819714471848
    3 -13.8513716980756
    3 -18.7944169895371
    3 -2.17430874576158
    3 -16.5346733609058
    };
    \addplot [semithick, red]
    table {%
    -0.5 28.6043838922666
    3.5 28.6043838922666
    };
    \addplot [semithick, darkslategray61]
    table {%
    -0.4 -13.0558730299372
    0.4 -13.0558730299372
    };
    \addplot [semithick, darkslategray61]
    table {%
    0.6 18.6996572945657
    1.4 18.6996572945657
    };
    \addplot [semithick, darkslategray61]
    table {%
    1.6 20.2181499801056
    2.4 20.2181499801056
    };
    \addplot [semithick, darkslategray61]
    table {%
    2.6 21.4778487560043
    3.4 21.4778487560043
    };
    \end{groupplot}
    
    \end{tikzpicture}
    

==> assets/sandbox/newsvendor.tex <==
\begin{tikzpicture}

    \definecolor{crimson_}{RGB}{214,39,40}
    \definecolor{darkorange_}{RGB}{255,127,14}
    \definecolor{forestgreen_}{RGB}{44,160,44}
    \definecolor{steelblue_}{RGB}{31,119,180}
    
    \begin{axis}[
        numeric axis,
        xmode=log,
        ymode=log,
        xmin=10, xmax=1000,
        ymin=5e-5, ymax=1,
        legend style={at={(axis cs: 1000, 1)}, anchor=north west, draw=none, yshift=0pt, xshift=6pt},
        legend cell align={left},
        xlabel={$n$},
        ylabel={rel. suboptimality},
        width=0.75\columnwidth,
        height=0.5\columnwidth,
        crimson/.style={crimson_, dotted},
        darkorange/.style={darkorange_, dash dot},
        forestgreen/.style={forestgreen_, dashed},
        steelblue/.style={steelblue_},
    ]
    \addlegendimage{steelblue}
    \addlegendentry{SAA};
    \addlegendimage{darkorange}
    \addlegendentry{KL};
    \addlegendimage{forestgreen}
    \addlegendentry{TV};
    \addlegendimage{crimson}
    \addlegendentry{$\bar{\CVAR}$};

    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    1 0.0427393185024543
    1 1.1774188166677
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    3 0.00900109169594735
    3 0.604225558067011
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    6 0.00771784434693361
    6 0.330951704573417
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    12 0.00339632588610926
    12 0.330664236879712
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    23 0.00309905737914484
    23 0.0819165362674388
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    43 0.00114027670639448
    43 0.0307450657316225
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    81 0.000606464272269671
    81 0.0187486738392141
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    151 0.000319869685663905
    151 0.0110404567447549
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    284 8.1368765343604e-05
    284 0.00680723165642532
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    533 0.00011294293670833
    533 0.00271481611506724
    };
    \addplot [draw=steelblue_, fill=steelblue_, mark=-, only marks]
    table{%
    x  y
    1000 0.000174897171377154
    1000 0.00177607550119657
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    1 0.00153642918629806
    1 0.00153642960747421
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    3 0.00125419425118699
    3 0.00153642959395194
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    6 0.000533692547138379
    6 0.00153643075291372
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    12 0.000597306983360365
    12 0.00282829199151184
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    23 0.000467651125383755
    23 0.00183342366539514
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    43 0.000288197593468985
    43 0.00251428495836945
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    81 0.000118049505909281
    81 0.00303182006783911
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    151 0.000221174291643117
    151 0.00303798621808937
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    284 0.000470334745106654
    284 0.00264498229933965
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    533 0.000132566288831018
    533 0.00193569679658042
    };
    \addplot [draw=darkorange_, fill=darkorange_, mark=-, only marks]
    table{%
    x  y
    1000 7.66775446575752e-05
    1000 0.00146783727187932
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    1 0.00153642918266175
    1 0.001536429186476
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    3 0.00153642918386724
    3 0.0015364291864685
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    6 0.00153642918471266
    6 0.00153642918648414
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    12 0.00153642918421409
    12 0.0015364291864933
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    23 0.00153642918570537
    23 0.00153642918816048
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    43 0.00124400448904882
    43 0.00153642918779113
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    81 0.000171571213565175
    81 0.00153642918708956
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    151 0.000243712893697088
    151 0.00153642918689076
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    284 0.000447713160972432
    284 0.00153642918665597
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    533 0.000184040565666417
    533 0.00153642918650653
    };
    \addplot [draw=forestgreen_, fill=forestgreen_, mark=-, only marks]
    table{%
    x  y
    1000 7.99482155050235e-05
    1000 0.00153642918645819
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    1 0.00153642918623396
    1 0.00153642918648223
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    3 0.00153642918479623
    3 0.00153642918647867
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    6 0.00153642916077991
    6 0.00153642918647905
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    12 0.00153642918604967
    12 0.00153642918649724
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    23 0.00153642918580292
    23 0.00153642919263814
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    43 0.00124400449214051
    43 0.00153642918898364
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    81 0.00017157121328587
    81 0.00153642918677973
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    151 0.000243712894103835
    151 0.00153642918675175
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    284 0.00044771315976707
    284 0.00153642918658538
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    533 0.000204971627687063
    533 0.00153642918648529
    };
    \addplot [draw=crimson_, fill=crimson_, mark=-, only marks]
    table{%
    x  y
    1000 7.99482348563287e-05
    1000 0.00153642918647295
    };
    \addplot [steelblue]
    table {%
    1 0.0427393185024543
    1 1.1774188166677
    };
    \addplot [steelblue]
    table {%
    3 0.00900109169594735
    3 0.604225558067011
    };
    \addplot [steelblue]
    table {%
    6 0.00771784434693361
    6 0.330951704573417
    };
    \addplot [steelblue]
    table {%
    12 0.00339632588610926
    12 0.330664236879712
    };
    \addplot [steelblue]
    table {%
    23 0.00309905737914484
    23 0.0819165362674388
    };
    \addplot [steelblue]
    table {%
    43 0.00114027670639448
    43 0.0307450657316225
    };
    \addplot [steelblue]
    table {%
    81 0.000606464272269671
    81 0.0187486738392141
    };
    \addplot [steelblue]
    table {%
    151 0.000319869685663905
    151 0.0110404567447549
    };
    \addplot [steelblue]
    table {%
    284 8.1368765343604e-05
    284 0.00680723165642532
    };
    \addplot [steelblue]
    table {%
    533 0.00011294293670833
    533 0.00271481611506724
    };
    \addplot [steelblue]
    table {%
    1000 0.000174897171377154
    1000 0.00177607550119657
    };
    \addplot [steelblue]
    table {%
    1 0.971530247450662
    3 0.0312012045026059
    6 0.024983373597515
    12 0.0216336427248541
    23 0.0176705412790388
    43 0.00606389359342409
    81 0.00464700403215021
    151 0.00256218179467749
    284 0.00122866508143535
    533 0.000582085979920015
    1000 0.000544116988495632
    };
    \addplot [darkorange]
    table {%
    1 0.00153642918629806
    1 0.00153642960747421
    };
    \addplot [darkorange]
    table {%
    3 0.00125419425118699
    3 0.00153642959395194
    };
    \addplot [darkorange]
    table {%
    6 0.000533692547138379
    6 0.00153643075291372
    };
    \addplot [darkorange]
    table {%
    12 0.000597306983360365
    12 0.00282829199151184
    };
    \addplot [darkorange]
    table {%
    23 0.000467651125383755
    23 0.00183342366539514
    };
    \addplot [darkorange]
    table {%
    43 0.000288197593468985
    43 0.00251428495836945
    };
    \addplot [darkorange]
    table {%
    81 0.000118049505909281
    81 0.00303182006783911
    };
    \addplot [darkorange]
    table {%
    151 0.000221174291643117
    151 0.00303798621808937
    };
    \addplot [darkorange]
    table {%
    284 0.000470334745106654
    284 0.00264498229933965
    };
    \addplot [darkorange]
    table {%
    533 0.000132566288831018
    533 0.00193569679658042
    };
    \addplot [darkorange]
    table {%
    1000 7.66775446575752e-05
    1000 0.00146783727187932
    };
    \addplot [darkorange]
    table {%
    1 0.00153642928922227
    3 0.00153642934215864
    6 0.0015364277989004
    12 0.00153642839017806
    23 0.00153642876026575
    43 0.00104368353865881
    81 0.00111702554256859
    151 0.000831720097615802
    284 0.00121224517695683
    533 0.000780020127965327
    1000 0.000392397771817081
    };
    \addplot [forestgreen]
    table {%
    1 0.00153642918266175
    1 0.001536429186476
    };
    \addplot [forestgreen]
    table {%
    3 0.00153642918386724
    3 0.0015364291864685
    };
    \addplot [forestgreen]
    table {%
    6 0.00153642918471266
    6 0.00153642918648414
    };
    \addplot [forestgreen]
    table {%
    12 0.00153642918421409
    12 0.0015364291864933
    };
    \addplot [forestgreen]
    table {%
    23 0.00153642918570537
    23 0.00153642918816048
    };
    \addplot [forestgreen]
    table {%
    43 0.00124400448904882
    43 0.00153642918779113
    };
    \addplot [forestgreen]
    table {%
    81 0.000171571213565175
    81 0.00153642918708956
    };
    \addplot [forestgreen]
    table {%
    151 0.000243712893697088
    151 0.00153642918689076
    };
    \addplot [forestgreen]
    table {%
    284 0.000447713160972432
    284 0.00153642918665597
    };
    \addplot [forestgreen]
    table {%
    533 0.000184040565666417
    533 0.00153642918650653
    };
    \addplot [forestgreen]
    table {%
    1000 7.99482155050235e-05
    1000 0.00153642918645819
    };
    \addplot [forestgreen]
    table {%
    1 0.00153642918596928
    3 0.00153642918613266
    6 0.00153642918644751
    12 0.00153642918643778
    23 0.00153642918649718
    43 0.00153642918648719
    81 0.00153642918647327
    151 0.00153642918620687
    284 0.00153642918630074
    533 0.0012154283319447
    1000 0.000853607795473956
    };
    \addplot [crimson]
    table {%
    1 0.00153642918623396
    1 0.00153642918648223
    };
    \addplot [crimson]
    table {%
    3 0.00153642918479623
    3 0.00153642918647867
    };
    \addplot [crimson]
    table {%
    6 0.00153642916077991
    6 0.00153642918647905
    };
    \addplot [crimson]
    table {%
    12 0.00153642918604967
    12 0.00153642918649724
    };
    \addplot [crimson]
    table {%
    23 0.00153642918580292
    23 0.00153642919263814
    };
    \addplot [crimson]
    table {%
    43 0.00124400449214051
    43 0.00153642918898364
    };
    \addplot [crimson]
    table {%
    81 0.00017157121328587
    81 0.00153642918677973
    };
    \addplot [crimson]
    table {%
    151 0.000243712894103835
    151 0.00153642918675175
    };
    \addplot [crimson]
    table {%
    284 0.00044771315976707
    284 0.00153642918658538
    };
    \addplot [crimson]
    table {%
    533 0.000204971627687063
    533 0.00153642918648529
    };
    \addplot [crimson]
    table {%
    1000 7.99482348563287e-05
    1000 0.00153642918647295
    };
    \addplot [crimson]
    table {%
    1 0.00153642918644529
    3 0.00153642918641349
    6 0.00153642918631892
    12 0.00153642918647492
    23 0.00153642918648948
    43 0.00153642918654373
    81 0.00153642918647187
    151 0.0015364291863277
    284 0.00153642918636121
    533 0.00115537137974553
    1000 0.000853607784580731
    };
    \end{axis}
    
    \end{tikzpicture}
    

==> assets/svm-table-old.tex <==
\begin{tabular}{llllll}
    \toprule
    &  &  & SAA & TV & $\bar{\CVAR}$ \\
   $\varepsilon$ & $\sigma$ & $\lambda$ &  &  &  \\
   \midrule
   \multirow[t]{9}{*}{$0.05$} & \multirow[t]{3}{*}{$0.05$} & $10^2$ & $0.500\,(0.001)$ & $0.057\,(0.049)$ & $0.076\,(0.070)$ \\
   &  & $10^4$ & $0.459\,(0.070)$ & $0.074\,(0.046)$ & $0.106\,(0.056)$ \\
   &  & $10^6$ & $0.157\,(0.036)$ & $0.029\,(0.015)$ & $0.030\,(0.015)$ \\
   & \multirow[t]{3}{*}{$0.25$} & $10^2$ & $0.445\,(0.066)$ & $0.050\,(0.034)$ & $0.064\,(0.053)$ \\
   &  & $10^4$ & $0.071\,(0.036)$ & $0.028\,(0.015)$ & $0.019\,(0.010)$ \\
   &  & $10^6$ & $0.026\,(0.005)$ & $0.015\,(0.007)$ & $0.014\,(0.005)$ \\
   & \multirow[t]{3}{*}{$0.5$} & $10^2$ & $0.154\,(0.040)$ & $0.034\,(0.018)$ & $0.035\,(0.018)$ \\
   &  & $10^4$ & $0.038\,(0.019)$ & $0.020\,(0.007)$ & $0.020\,(0.007)$ \\
   &  & $10^6$ & $0.021\,(0.005)$ & $0.016\,(0.005)$ & $0.016\,(0.005)$ \\
   \midrule
%    \multirow[t]{9}{*}{$0.1$} & \multirow[t]{3}{*}{$0.05$} & $10^2$ & $0.500\,(0.001)$ & $0.107\,(0.101)$ & $0.111\,(0.106)$ \\
%    &  & $10^4$ & $0.459\,(0.070)$ & $0.097\,(0.101)$ & $0.118\,(0.098)$ \\
%    &  & $10^6$ & $0.157\,(0.036)$ & $0.040\,(0.023)$ & $0.038\,(0.022)$ \\
%    & \multirow[t]{3}{*}{$0.25$} & $10^2$ & $0.445\,(0.066)$ & $0.083\,(0.079)$ & $0.088\,(0.084)$ \\
%    &  & $10^4$ & $0.071\,(0.036)$ & $0.027\,(0.011)$ & $0.021\,(0.011)$ \\
%    &  & $10^6$ & $0.026\,(0.005)$ & $0.015\,(0.006)$ & $0.014\,(0.005)$ \\
%    & \multirow[t]{3}{*}{$0.5$} & $10^2$ & $0.154\,(0.040)$ & $0.040\,(0.022)$ & $0.042\,(0.024)$ \\
%    &  & $10^4$ & $0.038\,(0.019)$ & $0.021\,(0.008)$ & $0.021\,(0.008)$ \\
%    &  & $10^6$ & $0.021\,(0.005)$ & $0.016\,(0.005)$ & $0.016\,(0.005)$ \\
%    \midrule
   \multirow[t]{9}{*}{$0.2$} & \multirow[t]{3}{*}{$0.05$} & $10^2$ & $0.500\,(0.001)$ & $0.137\,(0.127)$ & $0.148\,(0.124)$ \\
   &  & $10^4$ & $0.459\,(0.070)$ & $0.125\,(0.130)$ & $0.137\,(0.129)$ \\
   &  & $10^6$ & $0.157\,(0.036)$ & $0.046\,(0.027)$ & $0.049\,(0.029)$ \\
   & \multirow[t]{3}{*}{$0.25$} & $10^2$ & $0.445\,(0.066)$ & $0.114\,(0.115)$ & $0.121\,(0.115)$ \\
   &  & $10^4$ & $0.071\,(0.036)$ & $0.030\,(0.014)$ & $0.027\,(0.017)$ \\
   &  & $10^6$ & $0.026\,(0.005)$ & $0.015\,(0.006)$ & $0.014\,(0.005)$ \\
   & \multirow[t]{3}{*}{$0.5$} & $10^2$ & $0.154\,(0.040)$ & $0.050\,(0.030)$ & $0.055\,(0.036)$ \\
   &  & $10^4$ & $0.038\,(0.019)$ & $0.023\,(0.008)$ & $0.022\,(0.008)$ \\
   &  & $10^6$ & $0.021\,(0.005)$ & $0.017\,(0.005)$ & $0.017\,(0.005)$ \\
   \bottomrule
   \end{tabular}

==> assets/table/svm-table.tex <==
% \begin{tabular}{llllll}
%     \toprule
%     &  &  & SAA & TV & $\bar{\CVAR}$ \\
%    $\delta$ & $\sigma$ & $\lambda$ &  &  &  \\
%    \midrule
%    \multirow[t]{9}{*}{$0.05$} & \multirow[t]{3}{*}{$0.05$} & $10^4$ & $0.438\,(0.048)$ & $0.140\,(0.137)$ & $0.135\,(0.082)$ \\
%    &  & $10^6$ & $0.168\,(0.056)$ & $0.025\,(0.011)$ & $0.027\,(0.013)$ \\
%    &  & $10^8$ & $0.044\,(0.012)$ & $0.015\,(0.005)$ & $0.018\,(0.005)$ \\
%    & \multirow[t]{3}{*}{$0.25$} & $10^4$ & $0.085\,(0.033)$ & $0.023\,(0.008)$ & $0.020\,(0.010)$ \\
%    &  & $10^6$ & $0.033\,(0.011)$ & $0.016\,(0.006)$ & $0.015\,(0.006)$ \\
%    &  & $10^8$ & $0.020\,(0.010)$ & $0.020\,(0.009)$ & $0.021\,(0.009)$ \\
%    & \multirow[t]{3}{*}{$0.5$} & $10^4$ & $0.047\,(0.018)$ & $0.020\,(0.010)$ & $0.020\,(0.008)$ \\
%    &  & $10^6$ & $0.025\,(0.009)$ & $0.022\,(0.011)$ & $0.022\,(0.011)$ \\
%    &  & $10^8$ & $0.028\,(0.013)$ & $0.029\,(0.013)$ & $0.027\,(0.013)$ \\
%    \midrule
%   \multirow[t]{9}{*}{$0.2$} & \multirow[t]{3}{*}{$0.05$} & $10^4$ & $0.438\,(0.048)$ & $0.208\,(0.113)$ & $0.207\,(0.118)$ \\
%    &  & $10^6$ & $0.168\,(0.056)$ & $0.036\,(0.019)$ & $0.043\,(0.023)$ \\
%    &  & $10^8$ & $0.044\,(0.012)$ & $0.016\,(0.007)$ & $0.018\,(0.007)$ \\
%    & \multirow[t]{3}{*}{$0.25$} & $10^4$ & $0.085\,(0.033)$ & $0.032\,(0.017)$ & $0.024\,(0.014)$ \\
%    &  & $10^6$ & $0.033\,(0.011)$ & $0.015\,(0.006)$ & $0.015\,(0.006)$ \\
%    &  & $10^8$ & $0.020\,(0.010)$ & $0.022\,(0.010)$ & $0.020\,(0.009)$ \\
%    & \multirow[t]{3}{*}{$0.5$} & $10^4$ & $0.047\,(0.018)$ & $0.024\,(0.008)$ & $0.021\,(0.009)$ \\
%    &  & $10^6$ & $0.025\,(0.009)$ & $0.021\,(0.011)$ & $0.020\,(0.010)$ \\
%    &  & $10^8$ & $0.028\,(0.013)$ & $0.028\,(0.013)$ & $0.028\,(0.013)$ \\
%    \bottomrule
%    \end{tabular}


   \begin{tabular}{llllll}
    \toprule
    &  &  & SAA & TV & $\bar{\CVAR}$ \\
   $\delta$ & $\sigma$ & $\lambda$ &  &  &  \\
   \midrule
   \multirow[t]{20}{*}{$0.01$} & \multirow[t]{4}{*}{$0.01$} & $10^4$ & $0.500\,(0.002)$ & $0.212\,(0.055)$ & $0.108\,(0.043)$ \\
    &  & $10^6$ & $0.471\,(0.050)$ & $0.152\,(0.184)$ & $0.066\,(0.023)$ \\
    &  & $10^8$ & $0.362\,(0.038)$ & $0.423\,(0.158)$ & $0.277\,(0.195)$ \\
    &  & $10^{10}$ & $0.081\,(0.033)$ & $0.035\,(0.019)$ & $0.072\,(0.040)$ \\
    & \multirow[t]{4}{*}{$0.05$} & $10^4$ & $0.474\,(0.052)$ & $0.109\,(0.135)$ & $0.080\,(0.037)$ \\
    &  & $10^6$ & $0.170\,(0.057)$ & $0.038\,(0.021)$ & $0.046\,(0.026)$ \\
    &  & $10^8$ & $0.053\,(0.020)$ & $0.018\,(0.008)$ & $0.018\,(0.008)$ \\
    &  & $10^{10}$ & $0.039\,(0.029)$ & $0.043\,(0.020)$ & $0.027\,(0.015)$ \\
    & \multirow[t]{4}{*}{$0.25$} & $10^4$ & $0.097\,(0.047)$ & $0.038\,(0.030)$ & $0.033\,(0.027)$ \\
    &  & $10^6$ & $0.042\,(0.012)$ & $0.016\,(0.003)$ & $0.016\,(0.003)$ \\
    &  & $10^8$ & $0.022\,(0.010)$ & $0.019\,(0.005)$ & $0.017\,(0.004)$ \\
    &  & $10^{10}$ & $0.067\,(0.082)$ & $0.084\,(0.128)$ & $0.033\,(0.021)$ \\
    & \multirow[t]{4}{*}{$0.5$} & $10^4$ & $0.055\,(0.021)$ & $0.020\,(0.005)$ & $0.020\,(0.005)$ \\
    &  & $10^6$ & $0.030\,(0.008)$ & $0.020\,(0.004)$ & $0.020\,(0.004)$ \\
    &  & $10^8$ & $0.023\,(0.008)$ & $0.024\,(0.007)$ & $0.023\,(0.007)$ \\
    &  & $10^{10}$ & $0.202\,(0.140)$ & $0.128\,(0.128)$ & $0.163\,(0.136)$ \\
    & \multirow[t]{4}{*}{$0.75$} & $10^4$ & $0.047\,(0.014)$ & $0.022\,(0.006)$ & $0.022\,(0.006)$ \\
    &  & $10^6$ & $0.031\,(0.011)$ & $0.026\,(0.008)$ & $0.026\,(0.008)$ \\
    &  & $10^8$ & $0.036\,(0.017)$ & $0.035\,(0.014)$ & $0.031\,(0.010)$ \\
    &  & $10^{10}$ & $0.302\,(0.149)$ & $0.273\,(0.134)$ & $0.249\,(0.134)$ \\
    \midrule
   \multirow[t]{20}{*}{$0.05$} & \multirow[t]{4}{*}{$0.01$} & $10^4$ & $0.500\,(0.002)$ & $0.256\,(0.103)$ & $0.146\,(0.054)$ \\
    &  & $10^6$ & $0.471\,(0.050)$ & $0.208\,(0.184)$ & $0.103\,(0.055)$ \\
    &  & $10^8$ & $0.362\,(0.038)$ & $0.418\,(0.176)$ & $0.192\,(0.164)$ \\
    &  & $10^{10}$ & $0.081\,(0.033)$ & $0.041\,(0.024)$ & $0.064\,(0.040)$ \\
    & \multirow[t]{4}{*}{$0.05$} & $10^4$ & $0.474\,(0.052)$ & $0.126\,(0.100)$ & $0.111\,(0.054)$ \\
    &  & $10^6$ & $0.170\,(0.057)$ & $0.052\,(0.035)$ & $0.052\,(0.041)$ \\
    &  & $10^8$ & $0.053\,(0.020)$ & $0.020\,(0.008)$ & $0.022\,(0.011)$ \\
    &  & $10^{10}$ & $0.039\,(0.029)$ & $0.027\,(0.013)$ & $0.022\,(0.017)$ \\
    & \multirow[t]{4}{*}{$0.25$} & $10^4$ & $0.097\,(0.047)$ & $0.045\,(0.038)$ & $0.038\,(0.035)$ \\
    &  & $10^6$ & $0.042\,(0.012)$ & $0.019\,(0.004)$ & $0.016\,(0.003)$ \\
    &  & $10^8$ & $0.022\,(0.010)$ & $0.019\,(0.004)$ & $0.018\,(0.003)$ \\
    &  & $10^{10}$ & $0.067\,(0.082)$ & $0.061\,(0.114)$ & $0.043\,(0.045)$ \\
    & \multirow[t]{4}{*}{$0.5$} & $10^4$ & $0.055\,(0.021)$ & $0.023\,(0.007)$ & $0.023\,(0.006)$ \\
    &  & $10^6$ & $0.030\,(0.008)$ & $0.020\,(0.003)$ & $0.020\,(0.004)$ \\
    &  & $10^8$ & $0.023\,(0.008)$ & $0.024\,(0.007)$ & $0.024\,(0.007)$ \\
    &  & $10^{10}$ & $0.202\,(0.140)$ & $0.145\,(0.110)$ & $0.114\,(0.110)$ \\
    & \multirow[t]{4}{*}{$0.75$} & $10^4$ & $0.047\,(0.014)$ & $0.022\,(0.005)$ & $0.022\,(0.006)$ \\
    &  & $10^6$ & $0.031\,(0.011)$ & $0.026\,(0.007)$ & $0.026\,(0.007)$ \\
    &  & $10^8$ & $0.036\,(0.017)$ & $0.035\,(0.016)$ & $0.031\,(0.010)$ \\
    &  & $10^{10}$ & $0.302\,(0.149)$ & $0.290\,(0.112)$ & $0.252\,(0.139)$ \\
    \midrule
   \multirow[t]{20}{*}{$0.1$} & \multirow[t]{4}{*}{$0.01$} & $10^4$ & $0.500\,(0.002)$ & $0.329\,(0.097)$ & $0.168\,(0.078)$ \\
    &  & $10^6$ & $0.471\,(0.050)$ & $0.301\,(0.215)$ & $0.142\,(0.077)$ \\
    &  & $10^8$ & $0.362\,(0.038)$ & $0.248\,(0.178)$ & $0.184\,(0.127)$ \\
    &  & $10^{10}$ & $0.081\,(0.033)$ & $0.042\,(0.026)$ & $0.057\,(0.033)$ \\
    & \multirow[t]{4}{*}{$0.05$} & $10^4$ & $0.474\,(0.052)$ & $0.154\,(0.093)$ & $0.145\,(0.075)$ \\
    &  & $10^6$ & $0.170\,(0.057)$ & $0.059\,(0.048)$ & $0.060\,(0.046)$ \\
    &  & $10^8$ & $0.053\,(0.020)$ & $0.022\,(0.011)$ & $0.021\,(0.012)$ \\
    &  & $10^{10}$ & $0.039\,(0.029)$ & $0.030\,(0.021)$ & $0.030\,(0.020)$ \\
    & \multirow[t]{4}{*}{$0.25$} & $10^4$ & $0.097\,(0.047)$ & $0.046\,(0.042)$ & $0.041\,(0.036)$ \\
    &  & $10^6$ & $0.042\,(0.012)$ & \ccell[gray]{0.9}{$0.015\,(0.003)$} & \ccell[gray]{0.9}{$0.015\,(0.003)$} \\
    &  & $10^8$ & $0.022\,(0.010)$ & $0.020\,(0.005)$ & $0.018\,(0.004)$ \\
    &  & $10^{10}$ & $0.067\,(0.082)$ & $0.076\,(0.119)$ & $0.037\,(0.039)$ \\
    & \multirow[t]{4}{*}{$0.5$} & $10^4$ & $0.055\,(0.021)$ & $0.025\,(0.009)$ & $0.024\,(0.009)$ \\
    &  & $10^6$ & $0.030\,(0.008)$ & $0.021\,(0.004)$ & $0.021\,(0.005)$ \\
    &  & $10^8$ & $0.023\,(0.008)$ & $0.024\,(0.007)$ & $0.024\,(0.007)$ \\
    &  & $10^{10}$ & $0.202\,(0.140)$ & $0.145\,(0.097)$ & $0.112\,(0.110)$ \\
    & \multirow[t]{4}{*}{$0.75$} & $10^4$ & $0.047\,(0.014)$ & $0.022\,(0.006)$ & $0.022\,(0.006)$ \\
    &  & $10^6$ & $0.031\,(0.011)$ & $0.026\,(0.007)$ & $0.026\,(0.007)$ \\
    &  & $10^8$ & $0.036\,(0.017)$ & $0.034\,(0.013)$ & $0.031\,(0.010)$ \\
    &  & $10^{10}$ & $0.302\,(0.149)$ & $0.286\,(0.127)$ & $0.257\,(0.144)$ \\
    \midrule
   \multirow[t]{20}{*}{$0.2$} & \multirow[t]{4}{*}{$0.01$} & $10^4$ & $0.500\,(0.002)$ & $0.361\,(0.079)$ & $0.235\,(0.094)$ \\
    &  & $10^6$ & $0.471\,(0.050)$ & $0.328\,(0.180)$ & $0.198\,(0.106)$ \\
    &  & $10^8$ & $0.362\,(0.038)$ & $0.217\,(0.131)$ & $0.184\,(0.083)$ \\
    &  & $10^{10}$ & $0.081\,(0.033)$ & $0.046\,(0.023)$ & $0.061\,(0.035)$ \\
    & \multirow[t]{4}{*}{$0.05$} & $10^4$ & $0.474\,(0.052)$ & $0.225\,(0.142)$ & $0.197\,(0.100)$ \\
    &  & $10^6$ & $0.170\,(0.057)$ & $0.074\,(0.050)$ & $0.075\,(0.051)$ \\
    &  & $10^8$ & $0.053\,(0.020)$ & $0.025\,(0.015)$ & $0.026\,(0.015)$ \\
    &  & $10^{10}$ & $0.039\,(0.029)$ & $0.033\,(0.023)$ & $0.036\,(0.026)$ \\
    & \multirow[t]{4}{*}{$0.25$} & $10^4$ & $0.097\,(0.047)$ & $0.049\,(0.044)$ & $0.045\,(0.040)$ \\
    &  & $10^6$ & $0.042\,(0.012)$ & $0.019\,(0.005)$ & $0.016\,(0.003)$ \\
    &  & $10^8$ & $0.022\,(0.010)$ & $0.017\,(0.004)$ & $0.017\,(0.004)$ \\
    &  & $10^{10}$ & $0.067\,(0.082)$ & $0.070\,(0.113)$ & $0.039\,(0.033)$ \\
    & \multirow[t]{4}{*}{$0.5$} & $10^4$ & $0.055\,(0.021)$ & $0.027\,(0.014)$ & $0.027\,(0.015)$ \\
    &  & $10^6$ & $0.030\,(0.008)$ & $0.021\,(0.005)$ & $0.020\,(0.005)$ \\
    &  & $10^8$ & $0.023\,(0.008)$ & $0.024\,(0.007)$ & $0.024\,(0.007)$ \\
    &  & $10^{10}$ & $0.202\,(0.140)$ & $0.186\,(0.144)$ & $0.112\,(0.101)$ \\
    & \multirow[t]{4}{*}{$0.75$} & $10^4$ & $0.047\,(0.014)$ & $0.022\,(0.005)$ & $0.022\,(0.006)$ \\
    &  & $10^6$ & $0.031\,(0.011)$ & $0.026\,(0.007)$ & $0.026\,(0.007)$ \\
    &  & $10^8$ & $0.036\,(0.017)$ & $0.033\,(0.012)$ & $0.031\,(0.010)$ \\
    &  & $10^{10}$ & $0.302\,(0.149)$ & $0.289\,(0.129)$ & $0.250\,(0.140)$ \\
    \midrule
   \multirow[t]{20}{*}{$0.25$} & \multirow[t]{4}{*}{$0.01$} & $10^4$ & $0.500\,(0.002)$ & $0.365\,(0.113)$ & $0.257\,(0.124)$ \\
    &  & $10^6$ & $0.471\,(0.050)$ & $0.359\,(0.170)$ & $0.228\,(0.133)$ \\
    &  & $10^8$ & $0.362\,(0.038)$ & $0.221\,(0.100)$ & $0.199\,(0.099)$ \\
    &  & $10^{10}$ & $0.081\,(0.033)$ & $0.053\,(0.030)$ & $0.070\,(0.044)$ \\
    & \multirow[t]{4}{*}{$0.05$} & $10^4$ & $0.474\,(0.052)$ & $0.243\,(0.141)$ & $0.224\,(0.133)$ \\
    &  & $10^6$ & $0.170\,(0.057)$ & $0.077\,(0.051)$ & $0.078\,(0.054)$ \\
    &  & $10^8$ & $0.053\,(0.020)$ & $0.026\,(0.017)$ & $0.026\,(0.016)$ \\
    &  & $10^{10}$ & $0.039\,(0.029)$ & $0.038\,(0.019)$ & $0.030\,(0.025)$ \\
    & \multirow[t]{4}{*}{$0.25$} & $10^4$ & $0.097\,(0.047)$ & $0.050\,(0.044)$ & $0.048\,(0.043)$ \\
    &  & $10^6$ & $0.042\,(0.012)$ & $0.019\,(0.004)$ & $0.016\,(0.003)$ \\
    &  & $10^8$ & $0.022\,(0.010)$ & $0.018\,(0.005)$ & $0.017\,(0.004)$ \\
    &  & $10^{10}$ & $0.067\,(0.082)$ & $0.054\,(0.067)$ & $0.038\,(0.024)$ \\
    & \multirow[t]{4}{*}{$0.5$} & $10^4$ & $0.055\,(0.021)$ & $0.029\,(0.015)$ & $0.028\,(0.016)$ \\
    &  & $10^6$ & $0.030\,(0.008)$ & $0.021\,(0.004)$ & $0.020\,(0.005)$ \\
    &  & $10^8$ & $0.023\,(0.008)$ & $0.024\,(0.007)$ & $0.023\,(0.007)$ \\
    &  & $10^{10}$ & $0.202\,(0.140)$ & $0.149\,(0.116)$ & $0.111\,(0.106)$ \\
    & \multirow[t]{4}{*}{$0.75$} & $10^4$ & $0.047\,(0.014)$ & $0.023\,(0.007)$ & $0.022\,(0.005)$ \\
    &  & $10^6$ & $0.031\,(0.011)$ & $0.026\,(0.007)$ & $0.026\,(0.007)$ \\
    &  & $10^8$ & $0.036\,(0.017)$ & $0.034\,(0.012)$ & $0.031\,(0.010)$ \\
    &  & $10^{10}$ & $0.302\,(0.149)$ & $0.267\,(0.124)$ & $0.236\,(0.137)$ \\
   \end{tabular}
   

==> assets/transform/transform.tex <==
\tikzset{
    add hatch/.style 2 args={
        pattern=hatch, 
        pattern color=#1, 
        hatch size=5pt, 
        hatch angle=#2,
        hatch line width=0.1pt
    }
}

\begin{tikzpicture}
    \definecolor{crimson}{RGB}{214,39,40}
    \definecolor{steelblue}{RGB}{31,119,180}

    \begin{scope}[scale=3.2]
        % \path [semithick, draw=steelblue, add hatch={steelblue}{0}]
        % (0.3334,0.0)
        % --(-0.5,0.0)
        % --(-0.25,0.433)
        % --(0.0833,0.433)
        % --cycle;

        % \path [draw=gray, add hatch={gray}{-60}]
        % (0.0,0.0)
        % --(-0.5,0.0)
        % --(-0.0833,0.722)
        % --(0.1667,0.2887)
        % --cycle;

        % \path [draw=black, add hatch={black}{60}]
        % (-0.3334,0.0)
        % --(0.5,0.0)
        % --(0.25,0.433)
        % --(-0.08333,0.433)
        % --cycle;

        \path [draw=gray, add hatch={gray!50!white}{-120}]
        (-0.41667,0.1443)
        --(0,0.866)
        --(0.25,0.433)
        --(0.08334,0.1443)
        --cycle;

        % \path [draw=gray, add hatch={gray}{120}]
        % (0.0,0.0)
        % --(0.5,0.0)
        % --(0.08334,0.722)
        % --(-0.1667,0.2887)
        % --cycle;

        % \path [draw=gray, add hatch={gray}{180}]
        % (-0.25,0.433)
        % --(0,0.866)
        % --(0.41667,0.1443)
        % --(-0.08333,0.14434)
        % --cycle;

        \path [semithick, draw=steelblue, fill=steelblue!30!white, fill opacity=0.6]
        (0.3334,0.0)
        --(-0.5,0.0)
        --(-0.25,0.433)
        --(0.0833,0.433)
        --cycle;

        \path [thick, draw=crimson, fill=crimson!30!white]
        (0.1667,0.2887)
        --(0.0833,0.1443)
        --(-0.08333,0.14434)
        --(-0.1667,0.2887)
        --(-0.08333,0.433)
        --(0.0833,0.433)
        --cycle;

        \node [align=center, text=crimson] (amb) at (0, 0.2887) {$\amb$};
        \node [above right, xshift=5pt, align=center, text=steelblue] (dist) at (-0.5, 0.0) {$\distort$};
        \node [below, yshift=-15pt, align=center, text=gray] (permute) at (0.0, 0.866) {$\pi(\distort)$};

        \path [draw=black, fill=none] (-0.5, 0.0) -- (0.5, 0.0) -- ( 0.0, 0.866) -- cycle;
    \end{scope}

    \coordinate (box-east) at (current bounding box.east);
    \coordinate (box-north east) at (current bounding box.north east);
    \coordinate (box-south east) at (current bounding box.south east);
    
    % \node[anchor=north west, xshift=1cm, text=steelblue] at (box-north east) {$\distort$};
    % \node[anchor=south west, xshift=1cm, text=crimson] at (box-south east) {$\amb$};
    \node[anchor=west, xshift=0.2cm, yshift=0.2cm] (a) at (box-east) {${\color{crimson}\amb} = \bigcap_{\pi \in \Pi^n} \pi({\color{steelblue}\distort})$};
    \node[anchor=north west, yshift=-0.1cm, align=left] (b) at (a.south west) {${\color{steelblue}\distort} = {\color{crimson}\amb} + \major{n}$};

    \draw [crimson, very thin, -{Latex[length=2mm]}] (amb.north) |- (a.west);
    \draw [steelblue, very thin, -{Latex[length=2mm]}] (dist.east) -| ([xshift=-0.7cm]b.west) -- (b.west);
\end{tikzpicture}

==> content-old/calibration.tex <==
\section{Calibrating Risk Functionals} \label{sec:calibration}
Previously, we showed that law-invariant, coherent risk measures $\rho$ are $\varepsilon$-calibrated with $\varepsilon = \prob[W \notin \distort]$. 
For certain risk measures, numerical procedures that compute $\prob[W \in \distort]$
are available. These are \emph{distortion risks}, the distortion set of which is \emph{simple} as specified below. 
We then introduce a modified $\CVAR$ risk of this type. Its single parameter is calibrated such that 
$\prob[W \notin \distort] \leq \varepsilon$ for some $\varepsilon$. 

Another wide class of law-invariant, coherent risk measures are the $\phi$-divergences. For these, exact numerical procedures are unavailable.
Instead, efficient sampling procedures to calibrate the $\phi$-divergence at some level $\varepsilon$ are derived.

The proofs in this section are deferred to \ilarxiv{\cref{app:calibraton}}\ilpub{\cite[App.~D]{TR}}. Since our contribution is focused on calibration, we omit details related to solving \cref{eq:robustified-erm} and
refer to \ilarxiv{\cref{app:conic-risk}}\ilpub{\cite[App.~E]{TR}} instead. 
Optimizing distortion risks \cite{Bertsimas2009b, Mehta2022} and $\phi$-divergences \cite{Ben-Tal2013, Chouzenoux2019} 
is studied extensively in literature after all.

\subsection{Distortion risk} \label{sec:calibration:a}
We consider \emph{simple} distortion sets, which are generated by one vector. 
That is $\distort = \mu_\uparrow + (\M^n)^\circ$ with $\mu_{\uparrow} \in \Delta^n \cap \M^n$. \cref{fig:graphical-equivalence} depicts one such set.
Simple distortion sets correspond to \emph{distortion risk measures} 
(also called \emph{spectral risk measures} \cite[\S6.3.4]{Shapiro2021}, \cite[\S2.4.2]{Pflug2007})
which are law-invariant, coherent and \emph{comonotonic} \cite[Def.~4.1]{Bertsimas2009b}.
\begin{proposition} \label{lem:simple-distortion}
    For simple distortion sets $\distort = \mu_{\uparrow} + (\M^n)^\circ$ with $\mu \in \Delta^n$, the associated risk measure $\rho$ given by \cref{eq:distortion-representation}
    is a \emph{distortion risk measure} \cite[Def.~4.5]{Bertsimas2009b} and
    \begin{equation} \label{eq:distortion-risk}
        \rho(X) = \<\mu_{\uparrow}, X_{\uparrow}\>.
    \end{equation}
\end{proposition}

The coverage probability of simple distortion sets is expressed in terms of order statistics.

\begin{corollary} \label{lem:order-statistics-bound}
    For simple distortion sets $\distort = \mu_{\uparrow} + (\M^n)^\circ$ with $\mu \in \Delta^n$, the coverage probability 
    \begin{equation} \label{eq:order-statistics-bound}
        \prob[W \in \distort] = \prob\left[\sum_{i=1}^{k} \mu_{(i)} \leq U_{(k)}, \, \forall k \in [n-1]\right],
    \end{equation}
    where $U_{(1)} \leq U_{(2)} \leq \dots \leq U_{(n-1)}$ are order statistics associated with the uniform distribution over $[0, 1]$. 
\end{corollary}

\begin{remark} \label{rem:order-statistics-bound}
Bounds like the one in \cref{lem:order-statistics-bound} have been extensively studied due to the link with the 
\emph{uniform empirical process} and Kolmogorov-Smirnov statistics \cite[\S1]{Shorack2009}. 
An efficient method for the computation of \cref{eq:order-statistics-bound} is given in \cite{Moscovich2020}.
\end{remark}

We now present an example of a distortion risk that can be calibrated efficiently.
\begin{example} \label{ex:cvar}
    For $\gamma \in [0, 1]$, consider the following:
    \begin{equation} \label{eq:biased-cvar}
        \bar{\CVAR}^\gamma_n[X] = \left( \tfrac{d}{n-1} - \gamma \right) X_{(d)} + \sum_{i=d+1}^{n-1} \tfrac{X_{(i)}}{n-1} + \gamma X_{(n)},
    \end{equation}
    which is a \emph{distortion risk} with $d = \lceil (n-1)\gamma\rceil$ and $\gamma \geq 1/(n-1)$. 
    It is a known bound for the mean \cite{Anderson1969}, relating directly to a one-sided Kolmogorov-Smirnov
    bound. In \ilarxiv{\cref{app:calibraton}}\ilpub{\cite[App.~D]{TR}} we also establish a novel link with the conditional value-at-risk, explaining 
    the notation $\bar{\CVAR}$. 

    The exact method described in \cref{rem:order-statistics-bound} is applicable to \cref{eq:biased-cvar} and enables computing $\varepsilon$ 
    for a given $\gamma$. This dependency is monotone, with $\gamma = 0, 1$ giving $\varepsilon = 1, 0$ respectively. So
    scalar root finders\footnote{We use \texttt{brentq} as implemented in \texttt{scipy~1.10.0}} can find $\gamma$ for a given value of $\varepsilon$. 

    Alternatively, asymptotic bounds for \cref{eq:order-statistics-bound} exist in literature. For sufficiently large $n$ \cite[Thm.~11.6.2]{Wilks1964}
    \begin{equation} \label{eq:asymptotic}
            \varepsilon = e^{-2 (n-1) \gamma^2} \quad \Leftrightarrow \quad \gamma = \sqrt{\tfrac{\log(1/\varepsilon)}{2n - 2}}.
    \end{equation}    
\end{example}


% \section{Calibrating Risk Functionals} \label{sec:calibration}
% In this section we describe how to find distortion sets $\distort$ satisfying \cref{eq:confidence-distortion}. 
% To do so we consider two classes of parametric distortion sets and the associated risk measures.
% In both cases the parameter such that \cref{eq:confidence-distortion} holds for some user selected $\varepsilon$ can be determined efficiently. 

% \subsection{distortion risk} \label{sec:calibration:a}
% We first start by considering a special type of distortion set $\distort$, for which $\prob[W \in \distort]$ can be evaluated exactly. 
% Specifically we consider \emph{simple} distortion sets, which are generated by one vector. 
% That is $\distort = \{\mu\} + (\M^n)^\circ$ with $\mu \in \Delta^n$. \cref{fig:graphical-equivalence} depicts one such set.
% Simple distortion sets correspond to \emph{distortion risk measures} 
% (also called \emph{spectral risk measures} \cite[\S6.3.4]{Shapiro2021}, \cite[\S2.4.2]{Pflug2007})
% which are law-invariant, coherent and \emph{comonotonic} \cite[Def.4.1]{Bertsimas2009b}.
% \begin{lemma} \label{lem:simple-distortion}
%     For simple distortion sets $\distort = \{\mu\} + (\M^n)^\circ$ with $\mu \in \Delta^n \cap \M^n$, the associated risk measure $\rho$ given by \cref{eq:distortion-representation}
%     is a \emph{distortion risk measure} \cite[Def.~4.5]{Bertsimas2009b} and
%     \begin{equation} \label{eq:distortion-risk}
%         \rho[X] = \<\mu, X_{\uparrow}\>.
%     \end{equation}
% \end{lemma}
% \begin{proof}
%     Note that $\<\mu + s, X_{\uparrow}\> \leq \<\mu, X_{\uparrow}\>$ for all $s \in (\M^n)^\circ$ since it is the polar cone of $\Re_{\uparrow}^n$. 
%     Hence the supremum in \cref{eq:distortion-representation} is achieved at $\mu$. The characterization of $\rho$ as a distortion risk measure
%     then follows from \cite[Thm.~4.2]{Bertsimas2009b} -- keeping in mind that their risk measures are defined as $X \mapsto \rho(-X)$,
%     where $\rho$ follows our convention (cf. \cite[Thm.~2.1]{Bertsimas2009b}).
% \end{proof}

% Simple distortion sets are not only interesting from a computational point of view -- several efficient optimization algorithms exist for them \cite{Mehta2022} --
% but also from the statistical point of view. Their coverage probability can be computed exactly by expressing it in 
% terms of order statistics. 

% \begin{lemma} \label{lem:order-statistics-bound}
%     For simple distortion sets $\distort = \{\mu\} + (\M^n)^\circ$ with $\mu \in \Delta^n$, the coverage probability 
%     \begin{equation} \label{eq:order-statistics-bound}
%         \prob[W \in \distort] = \prob\left[\sum_{i=1}^{k} \mu_i \leq U_{(k)}, \, \forall k \in [n-1]\right],
%     \end{equation}
%     where $U_{(1)} \leq U_{(2)} \leq \dots \leq U_{(n-1)}$ are order statistics associated with the uniform distribution over $[0, 1]$. 
% \end{lemma}
% \begin{proof}
%     We have $W \in \{\mu\} + (\M^n)^\circ$ iff. $W - \mu \in (\M^n)^\circ$. This holds iff, for all $k \in [2, n]$ (cf. \cref{lem:dual-monotone-cone})
%     \begin{align*}
%         \sum_{i=k}^n W_i - \mu_i \leq 0 \, \Leftrightarrow \, 1 - \sum_{i=k}^n \mu_i \leq 1 - \sum_{i=k}^n W_i.
%     \end{align*}
%     Note that $W \in \Delta^n$ and $\mu \in \Delta^n$. Hence the final statement holds iff 
%     \begin{equation*}
%         \sum_{i=1}^k \mu_i \leq \sum_{i=1}^k W_i, \quad \forall k \in [n-1].
%     \end{equation*}
%     The fact that $\sum_{i=1}^k W_i \deq U_{(k)}$ follows from \cite[\S6.4]{David2003}.
% \end{proof}

% \begin{remark} \label{rem:order-statistics-bound}
% Bounds like the one in \cref{lem:order-statistics-bound} have been extensively studied due to the link with the 
% \emph{uniform empirical process} and Kolmogorov-Smirnov statistics \cite[\S1]{Shorack2009}. 
% An efficient method for the computation of \cref{eq:order-statistics-bound} is given in \cite{Moscovich2020}.
% \end{remark}

% We can characterize the ambiguity set associated with a distortion risk as follows:
% \begin{proposition} \label{prop:distortion-ambiguity}
%     Take some distortion risk $\rho$ with $\distort \dfn \dom \rho^{\diamond} = \mu + (\M^n)^\circ$ for some $\mu \in \Delta^n \cap \Re_{\uparrow}^n$. 
%     Then the ambiguity set $\amb \dfn \dom \rho^*$ is given as:
%     \begin{align*}
%         \amb = \left\{ S \nu \colon S \one_d = \one_n, \trans{\one}_n S = c, S \geq 0 \right\},
%     \end{align*}
%     with $\nu \in \Re^d$ containing the $d \leq n$ unique elements of $\mu$ and $c \in \Re^d$ the number of copies of each element of $\nu$ in $\mu$. 
% \end{proposition}
% \begin{proof}
%     This follows from \cref{prop:fundamental-equivalence-lemma} and \cref{lem:simple-distortion-characterization}.
% \end{proof}

% So we can evaluate risk measures as support functions of the polyhedral ambiguity set described above. 

% One special distortion risk measure is the \emph{conditional value-at-risk}, which we characterize 
% in terms of \cref{eq:distortion-risk} below.
% \begin{lemma} \label{lem:cvar-rewritten}
%     Consider $\CVAR_{n}^{\gamma} \colon \Re^{n} \to \Re$ as
%     \begin{equation} \label{eq:cvar-definition}
%         \CVAR_{n}^{\gamma}[X] = \inf_{\tau} \left\{ \tau + \frac{1}{(1-\gamma) n} \sum_{i=1}^{n} [X_i - \tau]_+ \right\},
%     \end{equation}        
%     for $\gamma \in [0, 1]$. Then
%     \begin{equation*}
%         (1 - \gamma)\CVAR_n^{\gamma}[X] = \left( \frac{d}{n} - \gamma \right) X_{(d)} + \sum_{i=d+1}^{n} \frac{X_{(i)}}{n},
%     \end{equation*}
%     with $d \dfn \lceil n\gamma \rceil$ is a distortion risk. 
% \end{lemma}
% \begin{proof}
%     Consider the minimizers in the definition of $\CVAR$:
%     \begin{equation*}
%         \argmin_\tau \left\{ \tau + \frac{1}{(1-\gamma) n} \sum_{i=1}^{n} [X_i - \tau]_+ \right\}.
%     \end{equation*} 
%     By \cite[Thm.~1]{Rockafellar2000}, this set is a closed bounded interval with the left endpoint being
%     \begin{align*}
%         \VAR_{n}^{\gamma}[X] &\dfn \inf_x \{x \colon F_n(x) \geq \gamma\} \\
%                             &= \inf_x \left\{ x \colon \sum_{i=1}^{n }\bm{1}_{(-\infty, x]}(X_i) \geq \gamma n \right\} = X_{(d)},
%     \end{align*}
%     with $F_n$ the empirical cdf, the definition of which we plugged in for the second equality.
%     For the third equality note that the left-hand side counts the number of values $X_i$ smaller than or equal to $x$. 
%     Assume 
%     \begin{equation}
%         X_{(d-k-1)} < X_{(d-k)} = X_{(d-k+1)} = \dots = X_{(d)},
%     \end{equation}
%     for $k \geq 0$. Then clearly there are at least $d = \lceil n \gamma \rceil > n\gamma$ values smaller than or equal to $X_{(d-k)}$. 
%     or any $z < X_{(d-k)}$ meanwhile 
%     there are at most $d-k-1$ samples values than or equal. Hence 
%     $\VAR_{n}^{\gamma}[X] = X_{(d-k)} = X_{(d)}$. 

%     Plugging into the cost of \cref{eq:cvar-definition} gives 
%     \begin{align}
%         &X_{(d)} + \frac{1}{(1-\gamma) n} \sum_{i=1}^{n} [X_i - X_{(d)}]_+ \nonumber \\
%         &\quad = X_{(d)} + \frac{1}{(1-\gamma) n} \sum_{i=d + 1}^{n} (X_{(i)} - X_{(d)}),\label{eq:cvar-rewritten}
%     \end{align}
%     where we used $X_{(i)} \leq X_{(d)}$ for $i \leq d$. The stated result follows from some 
%     basic algebraic manipulation. Finally note that $d/n - \gamma = (\lceil n\gamma \rceil - n\gamma)/n \leq 1/n$. 
%     So the monotonicity constraint on $\mu$ in \cref{lem:simple-distortion} is also satisfied.
% \end{proof}

% So $\CVAR_n^\gamma$ has a simple distortion set as in \cref{lem:simple-distortion} with 
% $\mu = (0, \dots, 0, \lceil n\gamma \rceil / n - \gamma, 1/n, \dots, 1/n)$. We can define a
% similar distortion risk that treats $Z_{n} \geq \esssup[Z]$ in $\hat{Z} = (Z_i)_{i=1}^{n}$ differently compared to the other samples. 
% \begin{equation} \label{eq:anderson-bound}
%     \bar{\CVAR}_n^\gamma[\hat{Z}] \dfn (1-\gamma) \CVAR_{n-1}^\gamma[(Z_i)_{i=1}^{n-1}] + \gamma Z_{n}.
% \end{equation}
% The associated simple distortion set in \cref{lem:simple-distortion} has
% \begin{equation} \label{eq:anderson-bound-vertex}
%     \mu = \left(0, \dots, 0, \tfrac{\lceil (n-1)\gamma \rceil}{n-1} - \gamma, \tfrac{1}{n-1}, \dots, \tfrac{1}{n-1}, \gamma\right),
% \end{equation}
% where we need $\gamma \geq 1/(n-1)$ for $\mu \in \Delta^n \cap \M^n$ to hold. 


% The expression in \cref{eq:anderson-bound} has been used as a high confidence bound for the mean before. It was first discovered 
% by \cite{Anderson1969} and relates directly to the Kolmogorov-Smirnov statistic. It was not related to $\CVAR$ as in \cref{eq:anderson-bound} before however.

% \begin{proposition}[Anderson {\cite{Anderson1969}}] \label{prop:anderson}
%         Consider an \iid{} sample $\{Z_i\}_{i=1}^{n-1}$ from $Z$ with $Z_{n} \geq \esssup[Z]$ and cdf $F$. Then
%         \begin{equation} \label{eq:anderson}
%                 \prob\left[ \E[Z] \leq \bar{\CVAR}_n^\gamma[Z]  \right] \geq 1 - \varepsilon,
%         \end{equation}
%         with $d = \lceil n\gamma\rceil$, $\bar{\CVAR}_n^\gamma[Z]$ as in \cref{eq:anderson-bound} and with
%         \begin{equation} \label{eq:bound}
%         \varepsilon = \prob\left[\exists z \in (-\infty, \bar{Z}] \colon F_n(z) - \gamma > F(z)\right],
%         \end{equation}
%         where $F(z) \dfn \prob[Z \leq z]$ the cumulative distribution function (cdf) and $F_n(z) \dfn \sum_{i=1}^{n} \bm{1}_{(-\infty, z]}(Z_i) / (n)$
%         the empirical cdf.
% \end{proposition}

% \begin{remark} \label{rem:asymptotic}
%         For large $n$ an asymptotic bound for \cref{eq:order-statistics-bound} in the case of \cref{eq:anderson-bound-vertex}
%         is given as \cite[Thm.~11.6.2]{Wilks1964}
%         \begin{equation*}
%                 \varepsilon = e^{-2 (n-1) \gamma^2} \quad \Leftrightarrow \quad \gamma = \sqrt{\tfrac{\log(1/\varepsilon)}{2n - 2}}.
%         \end{equation*}
%         For small $n$ the previous method in \cref{rem:order-statistics-bound} is preferred. The dependency of 
%         $\gamma$ on the confidence level is logarithmic. Hence its choice will not affect the result much. The $1/\sqrt{n}$ 
%         also occurs in many other DRO schemes (cf. \cite[Lem.~1]{Duchi2021b}).
% \end{remark}

% Calibrating $\bar{\CVAR}_\gamma^n$ involves finding a $\gamma \in [0, 1]$ such that the right-hand side of
% \cref{eq:order-statistics-bound} (computed using \cite{Moscovich2020}) equals $1-\varepsilon$.
% For this, standard scalar root finders\footnote{We use \texttt{brentq} as implemented in \texttt{scipy 1.10.0}} can be used. 
% Alternatively \cref{rem:asymptotic} can be used to calibrate $\bar{\CVAR}_{\gamma}^n$ 
% to act as an asymptotic high-confidence upper bound for $\E[Z]$. 



\subsection{$\phi$-divergence risk} \label{sec:calibration:b}
The $\phi$-divergence \cite{Ben-Tal2013} between $\mu, \nu \in \Delta^n$ is defined as 
\begin{equation} \label{eq:phi-divergence}
    I_{\phi}(\mu, \nu) = \sum_{i=1}^{n} \nu_i \phi\left( \mu_i/\nu_i \right)
\end{equation}
where $\phi(t)$ is convex for $t \geq 0$, $0\phi(a/0) \dfn a \lim_{t\to\infty} \phi(t)/t$, 
$0\phi(0/0) \dfn 0$ and $\phi(1) = 0$. A (centered) $\phi$-divergence ambiguity set is then
\begin{equation} \label{eq:phi-ambiguity}
    \amb_{\alpha}^n \dfn \left\{ \mu \colon I_{\phi}^n(\mu) \dfn I_{\phi}(\mu, \one_n/n) \leq \alpha\right\},
\end{equation}
with $\one_n/n \dfn (1/n, \dots, 1/n)$. The distortion set associated with it is $\distort_{\alpha}^n \dfn \amb_{\alpha}^n + (\M^n)^\circ$,
by \cref{thm:distortion-representation}. The set $\amb_{\alpha}^n$ is clearly permutation invariant, since \eqref{eq:phi-divergence}
is when $\nu = \one_n/n$.

Calibration of the $\phi$-divergence risk corresponds to solving 
\begin{equation} \label{eq:scenario-program}
    \argmin_{\alpha \geq 0} \left\{ \alpha \colon \prob\left[ W \in \distort_{\alpha}^n \right] \geq 1 - \epsilon \right\}.
\end{equation}
Unlike in the previous section, the probability cannot be evaluated exactly. Instead we 
compute a sample approximation to \cref{eq:scenario-program} as follows:

\begin{theorem} \label{thm:divergence-bound}
    Let $\{W^{(i)}\}_{i=1}^m$ be an \iid{} sample uniformly from $\Delta^n$ and $\alpha_i \dfn ({I_{\phi}^n}^*)^\diamond(W^{(i)})$
    for $i \in [m]$ with associated order statistics $\alpha_{(1)} \leq \dots \leq \alpha_{(m)}$. Then, for some $\epsilon \in [0, 1]$ 
    and some $u \in [n]$, 
    \begin{equation*}
        \prob\left[ \prob\left[ ({I_{\phi}^n}^*)^\diamond(W) \leq \alpha_{(u)} \mid W^{(i)} \right] \geq 1 - \varepsilon \right] \geq 1 - \beta
    \end{equation*}
    with $\beta = I_{1-\varepsilon}(u, m-u+1)$ the regularized incomplete beta function (i.e., the cdf of a beta distribution) at level $1-\epsilon$.
\end{theorem}

In practice, sample $m$ values of $\alpha_i$ and sort them. 
For given $\beta$ and $\varepsilon$, take $u \in [n]$ such that $\beta = I_{1-\varepsilon}(u, m-u+1)$
or increase $m$ if no such $u$ exists. Then \cref{thm:divergence-bound} 
says $\rho$ with radius $\alpha_{(u)}$ is $\varepsilon$-calibrated with probability at least $1-\beta$. 

\begin{remark}
    Note that \cref{eq:scenario-program} can be viewed as a chance-constrained program. So instead of relying on classical bounds from order statistics
    as we did in the proof of \cref{thm:distortion-bound} in \ilarxiv{\cref{app:calibraton}}\ilpub{\cite[App.~D]{TR}},
    we could use \cite[Thm.~3.7]{Campi2018}. We evaluate $({I_{\phi}^n}^*)^\diamond(W)$ 
    with a modified \emph{pool adjacent violators (PAV)} algorithm, which has worst-case computational complexity 
    of $\mathcal{O}(n)$ \cite{Best2000}. Details are provided in \ilarxiv{\cref{rem:pav}}\ilpub{\cite[Rem.~D.3]{TR}}.
\end{remark}

% For the sake of making the sample approximations computationally efficient we need the following.
% \begin{proposition} \label{prop:phi-containment}
%     Consider a $\phi$-distortion set $\distort_{\alpha}^n \dfn \amb_{\alpha}^n + (\M^n)^\circ$ with $\amb_{\alpha}^n$ as in \cref{eq:phi-ambiguity}. 
%     Then $\mu \in \distort_{\alpha}^n$ if and only if 
%     \begin{equation} \label{eq:phi-containment}
%         \left( {I_{\phi}^n}^* \right)^\diamond(\mu) = \sup_{\lambda \in \Re_{\uparrow}^n} \left\{ \sum_{i=1}^{n} \mu_i \cdot \lambda_i -  \frac{1}{n} \phi^*(\lambda_i) \right\}\leq \alpha.
%     \end{equation}
% \end{proposition}
% \begin{proof}
%     By construction of $\distort_{\alpha}^n = \amb_{\alpha}^n + (\M^n)^\circ$ we have $\mu \in \distort_{\alpha}^n$ 
%     if and only if there is some $s \in (\M^n)^\circ$ such that $\mu - s \in \amb_{\alpha}^n$ or 
%     \begin{align*}
%         \exists s \in (\M^n)^\circ\colon I_{\phi}^n(\mu - s) \leq \alpha \Leftrightarrow \inf_{s} \left\{ I_{\phi}^n(\mu - s) + \iota_{(\M^n)^\circ}(s) \right\} \leq \alpha.
%     \end{align*}
%     The infimum equals $I_{\phi}^n \episum \iota_{(\M^n)^\circ}$ by definition. 
%     Applying \cite[Thm.~11.23]{Rockafellar1998}, using $\dom I_{\phi}^n = \Delta^n$ and $\intr(\Delta^n) \cap (\M^n)^\circ \neq \emptyset$,
%     gives ${I_{\phi}^n} \episum \iota_{(\M^n)^\circ} = ({I_{\phi}^n}^* + \iota_{((\M^n)^\circ)^\circ})^* = ({I_{\phi}^n}^* + \iota_{(\Re^{n}_{\uparrow})})^*
%     = ({I_{\phi}^n}^*)^\diamond$, where we used \cite[Ex.~11.4]{Rockafellar1998} for the second equality.
%     For the equality in \cref{eq:phi-containment} we apply the tricks for the convex conjugate of a seperable sum and the conjugate of $\alpha f(x/\alpha)$
%     listed in \cite[App.~B, Table~3]{Beck2017}.
% \end{proof}

% \begin{remark}
%     To compute the supremum in \cref{eq:phi-containment} we specialize\footnote{
%         All that was required to specialize the algorithm of \cite{Best2000} is to note that 
%         \begin{equation*}
%             \argmax_{\lambda \in \Re} \quad \sum_{i=p}^{q} \left(\frac{1}{n}\right) \phi^*(\lambda) - \mu_i \cdot \lambda = \partial \phi\left( \frac{n \bar{\mu}_{[p, q]}}{q-p} \right),
%         \end{equation*}
%         which follows from simple algebra and \cite[Prop.~11.3]{Rockafellar1998}.
%     } the pool adjacent violators (PAV) algorithm from \cite{Best2000}. 
%     This requires a partition of $[n]$ given as $\set{J}$ consisting of blocks $[p, q] \subseteq [n]$. 
%     Let $[p, q]^+$ denote the block starting with $q+1$ and $[p, q]^-$ the one ending at $p-1$.
%     If no $[p, q]^+$ or $[p, q]^-$ exists then the output is $\emptyset$. 
%     For $\lambda, \mu \in \Re^n$ let $\lambda_{[p, q]} = (\lambda_p, \dots, \lambda_q)$ and $\bar{\mu}_{[p, q]} = \sum_{i=p}^q \mu_i$. 
%     Using this notation \hyperref[alg:pav]{Alg.~\ref{alg:pav}} computes the $\argmax$ of \cref{eq:phi-containment}. We give expressions for $\partial \phi$ 
%     for some $\phi$-divergences in \cref{tab:phi-table}.

%     {\SetAlgoNoLine\begin{algorithm}
%         \caption{The PAV algorithm for computing \cref{eq:phi-containment}}\label{alg:pav}
%         \textbf{initialization}: \\
%         \quad pick a partition $\set{J} \gets \{[i, i]\}_{i=1}^{n}$ \\
%         \quad\,\, let $\lambda_{[i, i]}^\star \in \partial \phi(n \bar{\mu}_{[i, i]})$ and $[p, q] \gets [1, 1]$.

%         \While{$[p, q]^+ \neq \emptyset$}{
%             \eIf{$\lambda^\star_{[p, q]} > \lambda^\star_{[p, q]^+}$}{
%                 \vspace{3pt}$J \gets (J \setminus \{[p, q], [p, q]^+\}) \cup ([p, q] \cup [p, q]^+)$ and $[p, q] \gets [p, q] \cup [p, q]^+$.\\
%                 let $\lambda_{[p, q]}^{\star} \in \partial \phi(n \bar{\mu}_{[p, q]}/(q-p))$.
%             }{
%                 $J \gets (J \setminus \{[p, q]^{-}, [p, q]\}) \cup ([p, q]^{-} \cup [p, q])$ and $[p, q] \gets [p, q]^{-} \cup [p, q]$.\\
%                 let $\lambda_{[p, q]}^{\star} \in \partial \phi(n \bar{\mu}_{[p, q]}/(q-p))$.                
%             }
%         }
%         \textbf{return}: $\lambda^\star$.\vspace{7pt}
%     \end{algorithm}}

%     Keeping these tools in mind, calibration of the $\phi$-divergence risk corresponds to solving 
%     \begin{equation} \label{eq:scenario-program}
%         \argmin_{\alpha \geq 0} \left\{ \alpha \colon \prob\left[ \left( {I_{\phi}^n}^* \right)^\diamond(W) \leq \alpha\right] \geq 1 - \epsilon \right\}.
%     \end{equation}
%     Letting $F_{\phi}$ denote the cdf of $({I_{\phi}^n}^*)^\diamond(W)$ then we can express this as $\alpha = F^{-1}_{\phi}(1-\epsilon)$.
%     That is we want to compute the quantile of a scalar random variable. 

%     \begin{theorem} \label{thm:divergence-bound}
%         Let $\{W^{(i)}\}_{i=1}^m$ be an \iid{} sample uniformly from $\Delta^n$ and $\alpha_i \dfn ({I_{\phi}^n}^*)^\diamond(W^{(i)})$
%         for $i \in [m]$ with associated order statistics $\alpha_{(1)} \leq \dots \leq \alpha_{(m)}$. Then, for some $\epsilon \in [0, 1]$ 
%         and some $u \in [n]$, 
%         \begin{equation*}
%             \prob\left[ \prob\left[ ({I_{\phi}^n}^*)^\diamond(W) \leq \alpha_{(u)} \mid W^{(i)} \right] \geq 1 - \epsilon \right] \geq 1 - \beta
%         \end{equation*}
%         with $\beta = I_{1-\epsilon}(u, m-u+1)$ the regularized incomplete beta function (i.e., the cdf of a beta distribution) at level $1-\epsilon$.

%         % Moreover 
%         % \begin{equation*}
%         %     \prob\left[ ({I_{\phi}^n}^*)^\diamond(W) \leq \alpha_{(u)} \right] \geq 
%         % \end{equation*}
%     \end{theorem}
%     \begin{proof}
%         The one-sided bound is stated in \cite[\S{}G.2.1]{Meeker2017}.% and the second in \cite[\S{}G.4.2]{Meeker2017}. 
%     \end{proof}

%     \begin{remark}
%         Note that \cref{eq:scenario-program} can be viewed as a scenario program. So instead of relying on classical bounds from order statistics,
%         we could use \cite[Thm.~3.7]{Campi2018}. 
%     \end{remark}

%     % The ordered conjugate is often more complex to compute analytically compared to the convex conjugate. However, efficient numerical procedures are available
%     % for convex seperable functions. 
    
%     % Specifically let $\varphi(x) = \sum_{i=1}^{n} f(x_i)$. Then
%     % \begin{equation*}
%     %     \begin{alignedat}{2}
%     %         -\varphi^{\diamond}(y) = &\min_{x \in \Re^n} & \quad &\sum_{i=1}^{n} f(x_i) - \<y_i, x_i\> \\
%     %                               &\sttshort & & x_1 \leq x_2 \leq \dots \leq x_n.
%     %     \end{alignedat}
%     % \end{equation*}
%     % The cost of the problem is separable and convex in terms of $x$. The monotonicity constraint (or simple chain constraint)
%     % is common in literature. Specifically \cite{Best2000} describes an algorithm of worst-case complexity $\mathcal{O}(n)$
%     % referred to as the pool adjacent violators (PAV) algorithm. To implement PAV one needs to evaluate 
%     % \begin{equation*}
%     %     \argmax_{x} yx - f^*(x) = \partial f(y).
%     % \end{equation*}
%     % We state these minimizers for the problem in \cref{prop:phi-containment} for several $\phi$-divergences in \cref{tab:phi-table} below.
% \end{remark}

% \begin{table*}
%     \begin{tabular}[t]{>{\bfseries}l c c c}
%         \toprule
%         Divergence & $\phi(t)$ & $\phi^{*}(\lambda)$ & $\partial \phi(t)$ \\
%         \midrule
%         Kullback-Leibler        & $t\log t - t + 1$     & $e^\lambda - 1$                           & $\log(t)$ \\
%         Burg Entropy            & $t-\log t - 1$        & $-\log(1-\lambda), \lambda < 1$           & $1 - t^{-1}$ \\
%         Hellinger distance      & $(\sqrt{t} - 1)^2$    & $\lambda/(1-\lambda), \lambda < 1$        & $1 - 1/\sqrt{t}$ \\
%         $\chi^2$-distance       & $(t-1)^2/t$           & $2 - 2\sqrt{1-\lambda}, \lambda < 1$      & $1 - t^2$ \\
%         Variation distance      & $|t-1|$               & $\max(-1, \lambda), \lambda < 1$          & $\begin{cases}-1, & t < 1 \\ [-1, 1], & t = 1 \\ \phantom{-}1, & 1 < t \end{cases}$ \\
%         \bottomrule
%     \end{tabular}
%     \centering
%     \caption{Some $\phi$-divergences, their conjugates and subgradients required for PAV.} \label{tab:phi-table}
% \end{table*}

% \section{Statistical Framework}
% We assume all random variables are defined on a sample space $(\Omega, \F, \prob)$ and consider $Z \colon \Omega \to (-\infty, \bar{Z}]$ 
% with $n$ iid. copies $\{Z_i\}_{i=1}^{n}$. These samples serve to model $\ell(\theta, \xi_i)$ for a fixed value of $\theta$,
% while $\bar{Z}$ replaces $\bar{\ell}(\theta)$. Under this setting we are interested in bounding the mean $\E[Z]$. 

% To do so we use the following:
% \begin{proposition}[Anderson {\cite{Anderson1969}}] \label{prop:anderson}
%         Let $Z \colon \Omega \to (-\infty, \bar{Z}]$ with sample $\{Z_i\}_{i=1}^{n}$. Then
%         \begin{equation} \label{eq:anderson}
%                 \prob\left[ \E[Z] \leq \left(\frac{d}{n} - \gamma \right) Z_{(d)} + \sum_{i=d+1}^{n} \frac{Z_{(i)}}{n} + \gamma \bar{Z}  \right] \geq 1 - \varepsilon,
%         \end{equation}
%         with $d = \lceil n\gamma\rceil$, $Z_{(1)} \leq \dots \leq Z_{(n)}$ the order statistics associated with the sample and for
%         \begin{equation} \label{eq:bound}
%         \varepsilon = \prob\left[\exists z \in (-\infty, \bar{Z}] \colon F_n(z) - \gamma > F(z)\right],
%         \end{equation}
%         where $F(z) \dfn \prob[Z \leq z]$ the cumulative distribution function (cdf) and $F_n(z) \dfn \sum_{i=1}^{n+1} \bm{1}_{(-\infty, z]}(Z_i) / (n+1)$
%         the empirical cdf, with $Z_{i+1} = \bar{Z}$ for notational convenience
% \end{proposition}

% \begin{remark}
%         The value \cref{eq:bound} is related to one-sided Kolmogorov-Smirnov statistics and is independent of the distribution of $Z$ when $F$
%         is continuous (cf. \cite[\S1]{Shorack2009}).

%         For an analytic expression for \cref{eq:bound}, see \cite[Thm.~9.1.1]{Shorack2009} or \cite[Thm.~11.6.1]{Wilks1964}. Such expressions are 
%         however numerically unstable. Instead we use the scheme proposed in \cite{Moscovich2020}, which is both numerically stable 
%         and has computational complexity $\mathcal{O}(n^2)$. To the authors knowledge this is the best available.

%         Also note that $\varepsilon$ is clearly non-increasing $\gamma$ with $\epsilon = 0$ and $\epsilon = 1$ for $\gamma = 1$ and $-1$ respectively. 
%         So we invert it using standard root finders\footnote{We use \texttt{brentq} as implemented in \texttt{scipy 1.10.0}}.
% \end{remark}

% \begin{remark}
%         For large $n$ an asymptotic bound for \cref{eq:bound} is given as \cite[Thm.~11.6.2]{Wilks1964}
%         \begin{equation*}
%                 \varepsilon = e^{-2n \gamma^2} \quad \Leftrightarrow \quad \gamma = \sqrt{\frac{\log(1/\varepsilon)}{2n}}.
%         \end{equation*}
%         Due to inaccuracies for small $n$ the previous method is preferred. It is informative that the dependency of 
%         $\gamma$ on the confidence level is logarithmic. Hence its choice will not affect the result much. The $1/\sqrt{n}$ 
%         is also of note as it occurs in many DRO schemes (cf. \cite[Lem.~1]{Duchi2021b}).
% \end{remark}

% We now relate the bound in \cref{eq:anderson} to $\CVAR$. 
% \begin{lemma} \label{lem:cvar-rewritten}
%         Let $\CVAR_{n}^{\gamma}[Z]$ be defined as in \cref{eq:conditional-value-at-risk}. That is 
%         \begin{equation} \label{eq:cvar-definition}
%                 \CVAR_{n}^{\gamma}[Z] = \inf_{\tau} \left\{ \tau + \frac{1}{(1-\gamma) n} \sum_{i=1}^{n} [Z_i - \tau]_+ \right\},
%         \end{equation}
%         for a sample $\{Z_i\}_{i=1}^{n}$ of the random variable $Z$.         
%         Then
%         \begin{equation*}
%                 (1 - \gamma) \CVAR_n^{\gamma}[Z] = \left( \frac{d}{n} - \gamma \right) Z_{(d)} + \sum_{i=d+1}^{n} \frac{Z_{(i)}}{n},
%         \end{equation*}
%         with $d \dfn \lceil n\gamma \rceil$ and $Z_{(1)} \leq \dots \leq Z_{(n)}$ the order statistics. 
% \end{lemma}
% \begin{proof}
%         Consider the minimizers in the definition of $\CVAR$:
%         \begin{equation*}
%                 \argmin_\tau \left\{ \tau + \frac{1}{(1-\gamma) n} \sum_{i=1}^{n} [Z_i - \tau]_+ \right\}.
%         \end{equation*} 
%         By \cite[Thm.~1]{Rockafellar2000}, this set is a closed bounded interval with the left endpoint being
%         \begin{align*}
%                 \VAR_{n}^{\gamma}[Z] &\dfn \inf_z \{z \colon F_n(z) \geq \gamma\} \\
%                                      &= \inf_z \left\{ z \colon \sum_{i=1}^{n }\bm{1}_{(-\infty, z]}(Z_i) \geq \gamma n \right\} = Z_{(d)},
%         \end{align*}
%         with $F_n$ the empirical cdf, the definition of which we plugged in for the second equality.
%         For the third equality note that the left-hand side counts the number of samples $Z_i$ smaller than or equal to $z$. 
%         Assume 
%         \begin{equation}
%                 Z_{(d-k-1)} < Z_{(d-k)} = Z_{(d-k+1)} = \dots = Z_{(d)},
%         \end{equation}
%         for $k \geq 0$. Then clearly there are at least $d = \lceil n \gamma \rceil > n\gamma$ samples smaller than or equal to $Z_{(d-k)}$. For any $z < Z_{(d-k)}$ meanwhile 
%         there are at most $d-k-1$ samples smaller than or equal. Hence 
%         $\VAR_{n}^{\gamma}[Z] = Z_{(d-k)} = Z_{(d)}$. 

%         Plugging into the cost of \cref{eq:cvar-definition} gives 
%         \begin{align}
%                 &Z_{(d)} + \frac{1}{(1-\gamma) n} \sum_{i=1}^{n} [Z_i - Z_{(d)}]_+ \nonumber \\
%                 &\quad = Z_{(d)} + \frac{1}{(1-\gamma) n} \sum_{i=d + 1}^{n} (Z_{(i)} - Z_{(d)}),\label{eq:cvar-rewritten}
%         \end{align}
%         where we used $Z_{(i)} \leq Z_{(d)}$ for $i \leq d$. The stated result follows from some 
%         basic algebraic manipulation.
% \end{proof}

% Note that $\CVAR$ has often been written in terms of order statistics (e.g. \eqref{eq:cvar-rewritten} is identical to \cite[Eq.~32]{Chun2012}). The connection to \cref{eq:anderson}
% has not been made before to our knowledge. 

% \begin{theorem}
%         Let $Z \colon \Omega \to (-\infty, \bar{Z}]$ with sample $\{Z_i\}_{i=1}^{n}$ and $\CVAR_n^\gamma$
%         as in \cref{eq:cvar-definition}. Then 
%         \begin{equation} \label{eq:cvar-bound}
%                 \prob\left[ (1 - \gamma) \CVAR_{n}^{\gamma}[Z] + \gamma \bar{Z} \geq \E[Z] \right] \geq 1 - \varepsilon,
%         \end{equation}
%         with $\varepsilon$ as given in \cref{eq:bound}.
% \end{theorem}
% \begin{proof}
%         This follows from \cref{lem:cvar-rewritten} and \cref{prop:anderson}.
% \end{proof}

% Plugging in $Z = \ell(\theta, \xi)$ implies \cref{eq:confidence-guarantee} from the introduction.
% So the bound in \cref{eq:cvar-bound} serves as a good data-driven proxy cost that replaces the unknown expected risk. 



==> content-old/distortion.tex <==
\section{Distortion Representation} \label{sec:distortion-representation}
The notion of law-invariant, coherent risk measures has been studied in depth before 
(see \cite[\S6.3.5]{Shapiro2021}, \cite{Shapiro2013}, \cite{Bertsimas2009b} and references within). 
They are usually motivated through an axiomatic framework. Our interest originates from 
the fact that they are a class of risk measures that satisfy a representation like the supremum in \cref{eq:distortion-bound}.

In our setting risk measures are defined by considering 
a finite sample space $\Omega^n = \{\omega_1, \dots, \omega_n\}$ with distribution $\one_n/n = (1/n, \dots, 1/n)$ and $\sigma$-algebra $\F$. 
Then any random variable $X \colon \Omega^n \to \Re$ is uniquely characterized by some vector in $x = (X(\omega_i))_{i=1}^{n} \in \Re^n$. 
Its components will later encode the samples, similarly to $L(\theta)$ in \eqref{eq:robustified-erm}.
The underlying distribution encodes that the samples are exchangeable and has 
the consequence that identically distributed random variables are characterized as permutations (cf. \ilarxiv{\cref{app:distortion-representation}}\ilpub{\cite[App.~C]{TR}})
\begin{lemma} \label{lem:identically-distributed}
    Consider two random variables $X, Y \colon \Omega^n \to \Re$ with $x, y \in \Re^n$ their vector characterization. Then 
    \begin{equation*}
        X \deq Y \quad \Leftrightarrow \quad \exists \pi \in \Pi^n \colon x = \pi(y),
    \end{equation*}
\end{lemma}

We consider coherent risks, which can be represented as support functions \cite[\S6.3]{Shapiro2021}%\cite{Pichler2021}
\begin{proposition} \label{def:ambiguity}
    For a $\rho \colon \Re^n \to \Re$, let $\amb \dfn \dom\rho^*$ be the \emph{ambiguity set}. 
    Then $\rho$ is coherent iff
    \begin{equation} \label{eq:ambiguity-representation}
        \rho(X) = \sup_{\mu \in \amb} \, \<\mu, X\>
    \end{equation}
    for some non-empty, closed and convex $\amb \subseteq \Delta^n$.
    Moreover $\rho$ is also law-invariant (i.e. $\rho(X) = \rho(Y)$ if $X \deq Y$) 
    iff $\pi \amb = \amb$ for all $\pi \in \Pi^n$.
\end{proposition}

We provide a motivation for \cref{def:ambiguity} in terms of the usual 
definition of a coherent risk measure in \ilarxiv{\cref{app:distortion-representation}}\ilpub{\cite[App.~C]{TR}}.

We refer to \cref{eq:ambiguity-representation} as the \emph{ambiguity representation} and define an analogous 
\emph{distortion representation} using the domain of the \emph{ordered convex conjugate}:
\begin{equation} \label{eq:ordered-conjugate}
    \rho^\diamond(\mu) \dfn \sup_{X \in \Re^n_{\uparrow}} \left\{ \<\mu, X\> - \rho(X) \right\},
\end{equation}
which differs from $\rho^*$ as the supremum is taken over $\Re^n_{\uparrow}$. 

\begin{theorem} \label{thm:distortion-representation}
    For a law-invariant, coherent risk $\rho \colon \Re^n \to \Re$, let $\distort \dfn \dom\rho^\diamond$
    denote the \emph{distortion set}. Then
    \begin{equation} \label{eq:distortion-representation}
        \rho(X) = \sup_{\mu \in \distort} \, \<\mu, X_{\uparrow}\>
    \end{equation}
    for $\distort$ closed, convex,
    \begin{enumerate*}[(i)]
        \item $\one_n/n \in \distort$,
        \item $\distort + (\M^n)^\circ = \distort$,
        \item $\sum_{i=1}^{n} \mu_i = 1$ for all $\mu \in \distort$ and
        \item any $\mu$ s.t. $\pi(\mu) \in \distort$ for all $\pi \in \Pi_n$ is nonnegative.
    \end{enumerate*}

    Moreover, letting $\amb$ be as in \cref{def:ambiguity},
    \begin{align} \label{eq:distort-ambiguity-relation}
        \distort &= \amb + (\M^n)^\circ& \text{and}& &\amb &= \bigcap_{\pi \in \Pi^n} \pi\left( \distort \right).
    \end{align}
\end{theorem}
\begin{proof}
    We only derive a valid $\distort$ such that \cref{eq:distortion-representation} holds, as this is the main property 
    we require further on. From \cref{eq:ambiguity-representation}:
    \begin{equation*}
        \rho(X) = \sup_{\mu \in \amb} \<\mu, X\> = \sup_{\mu \in \amb} \<\mu, X_{\uparrow}\> = \sup_{\mu \in \amb + (\M^n)^\circ } \<\mu, X_{\uparrow}\>.
    \end{equation*}
    The second and third equality follow by permutation invariance and the definition of the polar cone respectively. 
    So $\amb + (\M^n)^\circ $ is valid. The rest is shown in \ilarxiv{\cref{app:distortion-representation}}\ilpub{\cite[App.~C]{TR}}.
\end{proof}

The full derivation of \cref{eq:distort-ambiguity-relation} in \ilarxiv{\cref{app:distortion-representation}}\ilpub{\cite[App.~C]{TR}} makes extensive use of 
the link between $\Pi^n$, $\Re_{\uparrow}^n$ and vector majorization \cite{Marshall2011}.
% stated in terms of a group-induced cone ordering \cite{Steerneman1990}. 


\begin{figure}
    \vspace{0.7em}
    \includegraphics{assets/transform-converted-to.pdf}
    \vspace{0.5em}
    \centering
    \caption{Graphical depiction of \cref{thm:distortion-representation} for $n = 3$.
    The intersection with the simplex $\Delta^n$ is shown.} \label{fig:graphical-equivalence} \vspace{-1.5em}
\end{figure}


A visualization of \cref{eq:distort-ambiguity-relation} is provided in \cref{fig:graphical-equivalence}.
We highlight the link with the supremum in \cref{eq:distortion-bound}. In fact, when $\distort = \dom\rho^\diamond$ 
it cannot be further increased in size. Any set $\distort'$ satisfying \cref{eq:distortion-representation}
would have to be a subset of $\distort$. So $\prob[W \in \distort]$ cannot be increased further for the given risk measure. 
Moreover $\distort$ is invariant under addition with $(\M^n)^\circ$ as required by \cref{eq:distortion-bound}.

We conclude this section with:
\begin{theorem} \label{thm:main-theorem}
    A law-invariant, coherent risk $\rho \colon \Re^n \to \Re$ is $\varepsilon$-calibrated as in \cref{eq:well-callibrated} with $\varepsilon = \prob[W \notin \distort  = \amb + (\M^n)^\circ]$
    for $W$ uniformly distributed over $\Delta^n$.
\end{theorem}
\begin{proof}
    This follows by combining \cref{eq:distortion-representation} with \cref{thm:distortion-bound}. 
\end{proof}

\cref{thm:main-theorem} is considered the main contribution of this work. 
In the next section we show how it can be used to calibrate several existing risk measures at a specified level $\varepsilon$. 

\begin{remark} \label{rem:robust-sample}
    In \cref{thm:main-theorem} it is assumed that $L(\theta)$ includes some $\bar{\ell}(\theta) \geq \esssup_{\xi \in \Xi} \ell(\xi, \theta)$. 
    In practice, this value can be difficult to compute. So in practice we often replace it with an additional sample. 
    % This heuristic is similar 
    % to the one used in the scenario approach \cite{Campi2018}. Its properties and associated guarantees will be studied in future work. 
\end{remark}



% \section{Distortion Representation} \label{sec:distortion-representation}
% We derive the distortion representation of law-invariant, coherent risk measures. It is analogous to the ambiguity
% set representation, but only exists under law-invariance. The distortion representation will cleanly interface with the 
% statistical framework from the next section. 

% In our setting risk measures are defined by considering 
% a finite sample space $\Omega^n = \{\omega_1, \dots, \omega_n\}$ with distribution $\one_n/n = (1/n, \dots, 1/n)$. 
% Then any random vector $X \colon \Omega^n \to \Re$ is uniquely characterized by some vector in $\Re^n$. 
% The support will later encode the samples. The underlying distribution encodes the 
% fact that the samples are exchangeable and has 
% the consequence that identically distributed random variables are characterized in terms of permutations.
% \begin{lemma} \label{lem:identically-distributed}
%     Consider two random variables $X, Y \in \Re^n$ with underlying measure $\one_n/n = (1/n, \dots, 1/n)$. Then 
%     \begin{equation*}
%         X \deq Y \quad \Leftrightarrow \quad \exists \pi \in \Pi^n \colon X = \pi(Y). 
%     \end{equation*}
% \end{lemma}
% \begin{proof}
%     Proof deferred to \cref{app:distortion-representation}.
% \end{proof}

% Throughout the rest of this section we view \cref{lem:identically-distributed} as a definition of $X \deq Y$. 
% We consider risk measures as $\rho \colon \Re^n \to \eRe$. 


% \newcommand{\cohasm}[1]{\hyperref[def:coh:#1]{\sc a\oldstylenums{#1}}}
% \begin{definition}[coherent risk] \label{def:coh}
%     Consider a real valued function $\rho \colon \Re^n \to \eRe$
%     that is proper \footnote{
%         That is $\rho(X) > -\infty$ for all $X \in \Re^n$ and the domain $\mathrm{dom}(\rho) \dfn \{X \in \Re^n \colon \rho(X) < +\infty\}$ is nonempty.
%     } and lsc.. Assume (for $X, Y \in \Re^n$):
%     \begin{enumeratass}
%         \item \emph{convex}: $\rho(\alpha X + (1-\alpha) Y) \leq \alpha \rho(X) + (1-\alpha) \rho(Y)$, $\forall \alpha \in [0, 1]$;\label{def:coh:1}
%         \item \emph{monotone}: if $Y \geq X$, then $\rho(Y) \geq \rho(X)$;\label{def:coh:2}
%         \item \emph{translation equivariance}: $\rho(X+a) = \rho(X) + a$, $\forall a \in \Re$;\label{def:coh:3}
%         \item \emph{pos. homogeneity}: if $t > 0$, then $\rho(tX) = t\rho(X)$;\label{def:coh:4}
%     \end{enumeratass}
%     then $\rho$ is a \emph{coherent risk measure}. Consider also
%     \begin{enumeratass}[resume]
%         \item \emph{law invariance}: if $X \deq Y$, then $\rho(Y) = \rho(X)$. \label{def:coh:5}
%     \end{enumeratass}
% \end{definition}
% The first four assumptions were considered in \cite[\S1]{Ruszczynski2006}, while \cohasm{5} is considered in 
% \cite[Def.~4.4]{Bertsimas2009b}. By \cref{lem:identically-distributed} it implies that $\rho(X) = \rho(\pi X)$ 
% for all $\pi \in \Pi^n$. 

% The convex conjugate $\rho^* \colon \Re^n \to \eRe$ of a risk measure is given as 
% \begin{equation} \label{eq:convex-conjugate}
%     \rho^*(\mu) = \sup_{X \in \Re^n} \left\{ \<\mu, X\> - \rho(X) \right\}.
% \end{equation}

% Its domain is affected by the assumptions in \cref{def:coh}. 
% \begin{proposition} \label{prop:conjugate-duality}
%     Suppose that $\rho \colon \Re^n \to \eRe$ is proper, lsc., and convex. Then, $\rho = \rho^{**}$
%     with $\amb \dfn \mathrm{dom}(\rho^*)$ a non-empty and convex set. Moreover
%     \begin{enumerate}[itemsep=0pt]
%         \item \cohasm{2} holds iff $\mu \geq 0$ for any $\mu \in \amb$; \label{prop:conjugate-duality:2}
%         \item \cohasm{3} holds iff $\sum_{i=1}^{n} \mu_i = 1$ for any $\mu \in \amb$; \label{prop:conjugate-duality:3}
%         \item \cohasm{4} holds iff $\amb$ is closed and \label{prop:conjugate-duality:4}
%         \begin{equation*}
%             \rho(X) = \sup_{\mu \in \amb} \, \<\mu, X\>, \quad \forall X \in \Re^n
%         \end{equation*}
%         \item \cohasm{5} holds iff $\rho^*(\pi \mu) = \rho^*(\mu)$ for all $\pi \in \Pi^n, \mu \in \Re^n$. \label{prop:conjugate-duality:5}
%     \end{enumerate}
%     We assumed the underlying measure of the random variables is $\one_n/n = (1/n, \dots, 1/n)$ for (iv). 
% \end{proposition}
% \begin{proof}
%     By \cite[Prop.~2.112]{Bonnans2000} $\rho^*$ is proper and convex. 
%     Hence its domain must be non-empty and convex. 
%     Now \emph{(i)}--\emph{(iii)} follows from \cite[Thm.~2.2]{Ruszczynski2006}. 

%     By \cref{lem:identically-distributed}, \cohasm{5} holds iff $\rho(\pi X) = X$ for all $\pi \in \Pi^n$. 
%     We first show that \cohasm{5} implies $\rho^*(\pi \mu) = \rho^*(\mu)$ for all $\pi \in \Pi^n$.
%     First note that 
%     \begin{align*}
%         &\sup_{X} \left\{ \<\mu, X\> - \rho(X) \right\} = \sup_{X} \left\{ \<\mu, \pi(X)\> - \rho(\pi(X)) \right\} \\
%         &\qquad = \sup_{X} \left\{ \<\pi^{-1}(\mu), X\> - \rho(X) \right\}
%     \end{align*}
%     Since $\{\pi^{-1} \colon \pi \in \Pi^n\} = \Pi^n$ we have shown $\rho^*(\pi \mu) = \rho^*(\mu)$ for all $\mu \in \Re^n$
%     and all $\pi \in \Pi^n$. For the reverse implication we can apply the same reasoning and using that $\rho = \rho^{**}$. 
%     Note that this result specializes \cite[Prop.~2]{Shapiro2013}.
% \end{proof}

% We have the following corollary.
% \begin{corollary} \label{cor:ambiguity}
%     Some risk $\rho \colon \Re^n \to \eRe$ is coherent iff 
%     \begin{equation} \label{eq:ambiguity-representation}
%         \rho(X) = \sup_{\mu \in \amb} \, \<\mu, X\>
%     \end{equation}
%     for some non-empty, closed and convex $\amb \subseteq \Delta^n$.
%     Moreover $\rho$ is also law-invariant iff $\pi \amb = \amb$ for all $\pi \in \Pi^n$. 
%     The set $\amb$ is referred to as the \emph{ambiguity set}. 
% \end{corollary}

% Everything above is a summary of existing characterizations of risk measures.
% These were developed based on the convex conjugate. We now re-derive similar properties based on a different 
% notion of a conjugate. Define the \emph{ordered conjugate} of $\rho \colon \Re^n \to \eRe$ as 
% \begin{equation} \label{eq:ordered-conjugate}
%     \rho^{\diamond}(\mu) \dfn \sup_{X \in \M^n} \left\{ \<\mu, X\> - \rho(X) \right\}.
% \end{equation}
% For this new conjugate we have an alternative to \cref{prop:conjugate-duality} that has law-invariance embedded into it.

% We first consider some properties of \cref{eq:ordered-conjugate} by relating it to an infimal convolution.
% \begin{lemma} \label{lem:infimal-convolution}
%     Given some proper, convex, lsc. and law-invariant risk measure $\rho \colon \Re^n \to \eRe$ and $(\M^n)^\circ \dfn (\M^n)^\circ$
%     the polar of the monotone cone. Then 
%     \begin{equation*}
%         \rho^{\diamond} = (\rho + \indi_{\M^n})^* = \cl(\rho^* \episum \indi_{(\M^n)^\circ}).
%     \end{equation*}
%     Moreover if $\dom(\rho) \cap \intr(\M^n) = \emptyset$ then the $\cl$ is spurious. 
%     We say $\rho$ is \emph{montone-proper} when this holds. 
% \end{lemma}
% \begin{proof}
%     The first equality holds by definition of the conjugate and the indicator. 
%     Suppose $\dom(\rho) \cap \M^n = \emptyset$. By law invariance and \cref{lem:identically-distributed} 
%     this implies $\rho(\pi(X)) = +\infty$ for all $X \in \M^n$ and $\pi \in \Pi^n$. So $\dom \rho = \emptyset$, contradicting 
%     properness of $\rho$. Hence $\dom(\rho) \cap \M^n \neq \emptyset$. The rest of the result then 
%     follows from \cite[thm.~11.23]{Rockafellar1998}, where we used $\indi_{\M^n}^* = \indi_{(\M^n)^\circ}$ (cf. \cite[Ex.~11.4]{Rockafellar1998}). 
% \end{proof}

% We relate the domain of $\rho^{\diamond}$ to that of $\rho^*$. 
% \begin{proposition} \label{prop:fundamental-equivalence-lemma}
%     Let $\rho \colon \Re^n \to \eRe$ be a monotone-proper, lsc., convex and law-invariant risk measure. 
%     Then
%     \begin{equation*}
%         \mathrm{dom}\left( \rho^{\diamond} \right) = \mathrm{dom}\left( \rho^* \right) + (\M^n)^\circ.
%     \end{equation*}
%     Moreover
%     \begin{equation*}
%         \mathrm{dom}\left( \rho^* \right) = \bigcap_{\pi \in \Pi^n} \pi\left( \mathrm{dom}\left( \rho^{\diamond} \right) \right).
%     \end{equation*}
% \end{proposition}
% \begin{proof}
%     The first result follows from \cref{lem:infimal-convolution} and \cite[Ex.~1.28]{Rockafellar1998}. %
%     % For the remainder let $\distort \dfn \mathrm{dom}\left( \rho^{\diamond} \right)$ and $\amb \dfn \mathrm{dom}\left( \rho^* \right)$.
%     % We first prove an auxiliary result:
%     % \begin{equation} \label{eq:cone-invariance}
%     %     \text{If } \mu \in \distort \text{ then } \mu - (\M^n)^\circ \subseteq \distort. 
%     % \end{equation}
%     % Note that, for $s \in (\M^n)^\circ$ implies 
%     % \begin{equation*}
%     %     \begin{alignedat}{1}
%     %     &\<s, X\> \geq 0, \, \forall X \in \M^n \,\Leftrightarrow \, \<\mu - s, X\> \leq \<\mu, X\>, \, \forall X \in \M^n\\
%     %     &\qquad                                   \Leftrightarrow \, \<\mu - s\> - \rho(X) \leq \<\mu, X\> - \rho(X), \, \forall X \in \M^n.
%     %     \end{alignedat}
%     % \end{equation*}
%     % Thus if $\mu \in \distort$ -- i.e. the supremum of the final expression is finite -- then $\mu - s \in \distort$. We have therefore shown \cref{eq:cone-invariance}. 
%     %
%     % Next we show $\distort \subseteq \amb - (\M^n)^\circ$. For any element $\nu \in \amb - (\M^n)^\circ$ we can pick some $\mu \in \amb$ 
%     % and some $s \in (\M^n)^\circ$ such that $\nu = \mu - s$ by construction. By permutation invariance of $\set{A}$ (cf. \cref{prop:conjugate-duality:5})
%     % we have $\mu_{\uparrow} \in \set{A}$. Hence 
%     % \begin{align*}
%     %     &\sup_{X \in \Re^n} \left\{ \<\mu_{\uparrow}, X\> - \rho(X) \right\} = \sup_{X \in \Re^n} \left\{ \<\mu_{\uparrow}, X_{\uparrow} \> - \rho(X) \right\} \\
%     %     &\qquad = \sup_{X \in \M^n} \left\{ \<\mu_{\uparrow}, X \> - \rho(X) \right\} = \rho^{\diamond}(\mu_{\uparrow})
%     % \end{align*}
%     % are all finite. For the first equality we used \cite[Prop.~6.A.3]{Marshall2011} which states $\<\mu_{\uparrow}, X\> \leq \<\mu_{\uparrow}, X_{\uparrow}\>$.
%     % For the second we used permutation invariance of $\rho$, which holds by assumption and by \cref{lem:identically-distributed}. 
%     % We have thus shown that $\mu_{\uparrow} \in \distort$. Hence, by \cref{eq:cone-invariance}, we have $\mu_{\uparrow} - (\M^n)^\circ \subseteq \distort$.
%     % Then, by \cref{lem:permutation-hull-contained}, $\hull(\{\pi(\mu) \colon \pi \in \Pi^n\}) - (\M^n)^\circ \subseteq \distort$.
%     % Since $s \in (\M^n)^\circ$ and $\mu \in \hull(\{\pi(\mu) \colon \pi \in \Pi^n\})$ we have shown $\nu = \mu - s \in \distort$. 
%     %
%     % To show $\amb - (\M^n)^\circ \subseteq \distort$ it is sufficient to prove $\amb \subseteq \distort$ by using \cref{eq:cone-invariance}. 
%     % This holds trivially since 
%     % \begin{equation*}
%     %     \sup_{X\in\Re^n} \left\{ \<\mu, X\> - \rho(X) \right\} \geq \sup_{X \in \M^n} \left\{ \<\mu, X\> - \rho(X) \right\}.
%     % \end{equation*}
%     % So whenever $\mu \in \amb$, which implies the left-hand side is finite, then the right-hand side is finite too. Thus $\mu \in \distort$. 
%     The second result follows from \cref{lem:inverse-cone-shift}. 
% \end{proof}


% We can use this lemma to generalize \cref{prop:conjugate-duality}. 
% \begin{proposition} \label{prop:ordered-conjugate-duality}
%     Suppose that $\rho \colon \Re^n \to \eRe$ is monotone-proper, lsc., law-invariant and convex. Then
%     $\distort \dfn \mathrm{dom}(\rho^\diamond)$ is a convex set such that $\distort \cap \M^n \neq \emptyset$. 
%     Moreover
%     \begin{enumerate}[itemsep=0pt]
%         \item If $\mu \in \distort$ then $\{\mu\} + (\M^n)^\circ \subseteq \distort$;
%         \item \cohasm{2} holds iff any $\mu$ s.t. $\pi(\mu) \in \distort$ for all permutations $\pi \in \Pi^n$
%         is nonnegative. 
%         \item \cohasm{3} holds iff $\sum_{i=1}^{n} \mu_i = 1$ for any $\mu \in \distort$; 
%         \item \cohasm{4} holds iff $\distort$ is closed and
%         \begin{equation*} 
%             \rho(X) = \sup_{\mu \in \distort} \, \<\mu, X_{\uparrow}\>, \quad \forall X \in \Re^n
%         \end{equation*}
%     \end{enumerate}
% \end{proposition}
% \begin{proof}
%     The fact that $\distort$ is convex and that \emph{(ii)} holds follow
%     directly from \cref{prop:fundamental-equivalence-lemma} and \cref{prop:conjugate-duality}. 
%     Similarly $\distort$ should contain all permutations of at least one vector $\mu$, since otherwise $\dom\rho^*$ is 
%     empty by \cref{prop:fundamental-equivalence-lemma}. This can only be the case when $\mu_{\uparrow} \in \distort$ by \cref{lem:opposite-hull-contained}. 
%     So $\distort \cap \M^n \neq \emptyset$. 

%     Meanwhile \emph{(i)} follows from \cref{prop:fundamental-equivalence-lemma}
%     and $(\dom \rho^* + (\M^n)^\circ) + (\M^n)^\circ = \dom \rho^* + (\M^n)^\circ$ since $(\M^n)^\circ$ is a convex cone.

%     Let $\bar{\rho} = \rho + \iota_{\Re^n}$ as in \cref{lem:infimal-convolution}.
%     Then $\distort = \mathrm{dom}(\bar{\rho}^*)$. 
%     By permutation invariance $\bar{\rho}(X_{\uparrow}) = \rho(X_{\uparrow}) = \rho(X)$ for all $X \in \Re^n$. 
%     We can then prove \emph{(iii)} by noting that $(X + a)_{\uparrow} = X_{\uparrow} + a$. 
%     Hence \cohasm{3} holds for $\bar{\rho}$
%     iff it holds for $\rho(X) = \bar{\rho}(X_{\uparrow})$. Thus we can apply \cref{prop:conjugate-duality:3} 
%     to $\bar{\rho}$ in order to link \cohasm{3} with $\mathrm{dom}(\rho^{\diamond}) = \mathrm{dom}(\bar{\rho}^{*})$. 
%     For \emph{(iv)} we use a similar argument noting that $(\alpha X)_{\uparrow} = \alpha X_{\uparrow}$ for all $X \in \Re^n$
%     and all $\alpha \geq 0$ and apply \cref{prop:conjugate-duality:4}. The only property of $\rho$ 
%     that does not transfer to $\bar{\rho}$ is monotonicity. So \emph{(ii)} is more complex. 
% \end{proof}

% We conclude with an anolog to \cref{cor:ambiguity}, defining the \emph{distortion representation} of a law-invariant, coherent risk measure.
% The relation with the ambiguity representation from \cref{prop:fundamental-equivalence-lemma} is presented graphically in \cref{fig:graphical-equivalence}.
% \begin{corollary}
%     Some risk $\rho \colon \Re^n \to \eRe$ is law-invariant and coherent iff 
%     \begin{equation} \label{eq:distortion-representation}
%         \rho(X) = \sup_{\mu \in \distort} \, \<\mu, X_{\uparrow}\>
%     \end{equation}
%     for a closed and convex \emph{distortion set} $\distort$ with
%     \begin{enumerate*}[(i)]
%         \item $\one_n/n \in \distort$;
%         \item $\mu + (\M^n)^\circ \subseteq \distort$ for all $\mu \in \distort$;
%         \item $\sum_{i=1}^{n} \mu_i = 1$;
%         \item any $\mu$ s.t. $\pi(\mu) \in \distort$ for all $\pi \in \Pi_n$ is nonnegative.
%     \end{enumerate*}
% \end{corollary}
% \begin{proof}
%     Any coherent risk measure has $\dom(\rho) = \Re^n$.
%     So $\rho$ is automatically monotone-proper. The other facts then follow from \cref{prop:ordered-conjugate-duality},
%     with the exception of \emph{(i)}.  
%     To prove this final fact note that for any $\mu \in \dom\rho^*$ we have $\hull(\{\pi(\mu) \colon \pi \in \Pi_n\}) \subseteq \dom \rho^*$,
%     by law-invariance and convexity. Let $E \in \Re^{n \times n}$ denote the matrix of all ones. 
%     Then $E\mu/n \in \hull(\{\pi(\mu) \colon \pi \in \Pi_n\})$. Since $\sum_{i=1}^{n} \mu_i = 1$ we have 
%     $E\mu/n = \one_n /n$. So if $\one_n /n \notin \dom \rho^*$ then $\dom \rho^*$ 
%     has to be empty by contradiction. Thus $\distort$ should contain $\one_n/n$ since otherwise $\dom\rho^* = \emptyset$ 
%     by \cref{prop:fundamental-equivalence-lemma}. 
% \end{proof}

% \begin{figure}
%     \input{assets/transform.tex}
%     \vspace{1em}
%     \centering
%     \caption{Graphical depiction of \cref{prop:fundamental-equivalence-lemma} for $n = 3$.
%     The intersection with the simplex $\Delta^n$ is shown. Let $\amb \dfn \mathrm{dom}(\rho^*)$, 
%     $\distort \dfn \mathrm{dom}(\rho^{\diamond})$.} \label{fig:graphical-equivalence}
% \end{figure}



==> content-old/intro.tex <==
\section{Introduction}
In this work we consider \emph{expected risk minimization}
\begin{equation} \label{eq:expected-risk-minimization}
    \begin{alignedat}{2}
        & \minimize_{\theta \in \Theta} &\quad& \E[ \ell(\theta, \xi)].
    \end{alignedat}
\end{equation}
Here $\Theta \subseteq \Re^{n_\theta}$ and $\xi \colon \Omega \to \Xi \subseteq \Re^{n_{\xi}}$ a random vector defined 
on sample space $(\Omega, \F, \prob)$. 
Problems like \cref{eq:expected-risk-minimization} are omnipresent in machine-learning and statistics \cite{Shalev-Shwartz2013,Vapnik1998}. 

In practice the expectation in \cref{eq:expected-risk-minimization} cannot be evaluated exactly. Instead 
a sample $\{\xi_i\}_{i=1}^n$ is available. Let $\ell_i(\theta) = \ell(\theta, \xi_i)$ and $L(\theta) = (\ell_1(\theta), \dots, \ell_{n}(\theta))$.
We then solve 
\begin{equation} \label{eq:robustified-erm}
    \begin{alignedat}{2}
        & \minimize_{\theta \in \Theta} \, \maximize_{\mu \in \amb} &\quad& \<\mu, L(\theta)\>,
    \end{alignedat}
\end{equation}
for some convex, non-empty and closed \emph{ambiguity set} $\amb \subset \Re^n$ of probability vectors. 
The usual \emph{empirical risk minimization} or \emph{sample average approach (SAA)} amounts to $\amb = \{\one_n/n\}$. 
We denote the value of the maximization in \cref{eq:robustified-erm} as $\rho[L(\theta)]$
and refer to it as a \emph{risk measure} \cite[\S6.3]{Shapiro2021}. When $\amb$ is permutation invariant 
(i.e. for any $\mu \in \amb$ and permutation $\pi$, $\pi\mu \in \amb$) we show
\begin{equation} \label{eq:well-callibrated}
    \prob\left[\rho[L(\theta)] \dfn \sup_{\mu \in \amb} \<\mu, L(\theta)\> \geq \E[\ell(\theta, \xi)]\right] \geq 1 - \varepsilon
\end{equation}
for all $\theta \in \Theta$ when $\ell_n(\theta)$ is replaced by $\bar{\ell}(\theta)$ which upper bounds $\ell(\theta, \xi)$ with probability one. 
The value of $1 - \varepsilon$ is given by the volume of a so-called \emph{distortion set}, which is related to $\rho$ through a modified convex conjugate. 
Whenever $\rho$ satisfies \cref{eq:well-callibrated} we say it is \emph{$\varepsilon$-calibrated}. Note that \cref{eq:well-callibrated} defines two problems:
\emph{(i)} an analysis problem, where given some $\rho$ a $\varepsilon$ should be determined; \emph{(ii)} a synthesis/calibration problem where we want to determine some (parametric) $\rho$
such that \cref{eq:well-callibrated} holds for some user provided $\varepsilon$. We solve both problems in this work and it turns out that calibrated risk measures solving \emph{(ii)} serve as 
good proxy costs for \cref{eq:expected-risk-minimization}. 

Solving \cref{eq:robustified-erm} instead of a sample average is nothing new and several sets $\amb$ have been considered under the framework of \emph{distributionally robust optimization (DRO)} \cite{Shapiro2021}.
Specifically $\amb$ can be based on moments as in \cite{Delage2010}, divergence from the empirical distribution as in \cite{Ben-Tal2013},
Wasserstein distance \cite{Esfahani2018b} or other statistical hypothesis tests \cite{Bertsimas2018}. See \cite{Lin2022,Rahimian2019} for recent surveys.
There are however some issues with classical DRO. Sets often depend on some parameters (e.g. some radius). These are sometimes determined using concentration inequalities \cite{Delage2010} 
or using inexact asymptotic bounds \cite{Ben-Tal2013} to make sure the true distribution is contained within $\amb$ with high confidence. This can often be 
conservative in the case fo concentration inequalities, either due to loose constants in the concentration inequalities or due to the shape of the ambiguity set. So instead one often resorts to either bootstrapping or 
cross validation (cf. \cite{Esfahani2018b}), which can be computationally expensive and lack statistical guarantees for finite samples, similarly to the asymptotic bounds. 

Recently, in the asymptotic setting, this conservativeness has been tackled by looking at \emph{cost-aware} bounds like \cref{eq:well-callibrated} \cite{Duchi2021b,Lam2019}
with good results. They also discuss the gap between \cref{eq:well-callibrated} and the usual uniform bounds (i.e. $\prob[\rho[L(\theta)] \geq \E[\ell(\theta, \xi)], \forall \theta] \geq 1 - \varepsilon'$)
provided by DRO. The finite sample case has not been considered much. We take the first steps in that direction in this work. 

To summarize, our approach is novel as follows:
\begin{enumerate}
    \item Our scheme provides \emph{cost-aware}, point-wise statistical guarantees as in \cref{eq:well-callibrated} for any number of samples;
    \item The bounds are tight for any distribution, 
            replacing the involved analytical derivations of concentration inequalities with efficient numerical procedures;
    \item The framework applies to many risks from literature, including distortion \cite{Bertsimas2009b} and $\phi$-divergence risks \cite{Ben-Tal2013};
    \item We present the \emph{distortion representation} of risks.
\end{enumerate}
The resulting scheme also outperforms SAA in both regression and classification as illustrated in \cref{sec:case-studies}, while being less sensitive to tuning parameters.

We exploit results from convex duality \cite{Rockafellar1998}, order statistics \cite{Wilks1964,David2003}, Kolmogorov-Smirnov statistics \cite{Moscovich2020}, 
majorization \cite{Marshall2011,Steerneman1990} and isotonic regression \cite{Best2000}. 








% The classical approach of \emph{empirical risk minimization}, where a cost $\sum_{i=1}^{n} \ell(\theta, \xi_i)/n$
% is minimized, often does not suffice due to the well known problem of over-fitting. Instead \emph{distributionally robust optimization (DRO)} 
% or \emph{risk averse stochastic programming} has been considered recently. Here, one minimizes a cost 
% \begin{equation} \label{eq:ambiguity-representation-continuous}
%     \rho[\ell(\theta, \xi)] = \sup_{\mu \in \set{A}} \int \ell(\theta, \xi) \di \mu(\xi). 
% \end{equation}
% The function $\rho$, referred to as a \emph{risk measure}, maps (scalar) random variables to real values and is \emph{coherent} whenever the \emph{ambiguity set} $\set{A}$ is a non-empty, closed and 
% convex set of probability distributions \cite{Ruszczynski2006}. 

% In classical DRO, the ambiguity set is calibrated such that 
% \begin{equation}
%     \prob[\mu_{\star} \in \amb] \geq 1 - \varepsilon,
% \end{equation}
% with $\mu_{\star}$ the true distribution of $\xi$. Such sets can be based on moments \cite{Delage2010}, divergence from the empirical distribution \cite{Ben-Tal2013},
% Wasserstein distance \cite{Esfahani2018b} or other statistical hypothesis tests \cite{Bertsimas2018}. 
% If this distribution is within $\amb$ then clearly the maximum is larger than $\E[\ell(\theta, \xi)]$ 
% uniformly over $\theta$. That is 
% \begin{equation} \label{eq:uniform-confidence-guarantee}
%     \prob\left[\rho[\ell(\theta, \xi)] \geq \E[\ell(\theta, \xi)], \forall \theta \in \Theta\right] \geq 1 - \varepsilon.
% \end{equation}
% As previously observed in \cite{Duchi2021b,Lam2019}, guaranteeing that $\mu_{\star} \in \mathcal{A}$ can be overly conservative.
% This is why, in practice, the ambiguity set $\amb$ is either calibrated 
% using bootstrapping \cite{Delage2010}, asymptotic versions of \cref{eq:uniform-confidence-guarantee} \cite{Bertsimas2018, Ben-Tal2013} or using cross-validation \cite{Esfahani2018b}. 
% These methods are either computationally expensive or lack guarantees for low sample counts -- the case where over-fitting is likely to occur.

% Instead it can be helpful to initially focus on a point-wise guarantee instead of the uniform one of \cref{eq:uniform-confidence-guarantee}. 
% That is 
% \begin{equation} \label{eq:point-confidence-guarantee}
%     \prob[\rho[\ell(\theta, \xi)] \geq \E[\ell(\theta, \xi)]] \geq 1 - \varepsilon, \quad \forall \theta \in \Theta.
% \end{equation}
% This is the approach of \cite{Duchi2021b,Lam2019}. 
% They start with a DRO scheme based on $\phi$-divergence balls for $\amb$, guaranteeing \cref{eq:point-confidence-guarantee} in the limit $n \to \infty$. They show that a slight 
% increase in the radius of the ball $\amb$ suffices when both sides of the event in \cref{eq:point-confidence-guarantee} are minimized over $\theta$. 
% These guarantees however only hold for sufficiently large $n$. So over-fitting can still occur.% (cf. Figure~1(b) in \cite{Duchi2021b}). 

% We similarly produce guarantees like \cref{eq:point-confidence-guarantee}, but ours are applicable for any number of samples. 
% To do so we begin by providing an alternative representation of \cref{eq:ambiguity-representation-continuous} when the 
% distributions are only supported on the samples and when the risk measure is \emph{law-invariant}. That is, it produces the same result for
% identically distributed random variables. We call this alternative representation a \emph{distortion representation}, which
% relates to distortion risk measures \cite{Bertsimas2009b} and involves a modified support function over a \emph{distortion set}. 

% Results from order statistics then enable computing $\varepsilon$ in \cref{eq:point-confidence-guarantee} 
% for any such risk measure in terms of the volume of the distortion set. 
% For a subset of these risk measures we conversely illustrate how, given some $\varepsilon$,
% the risk measure can be configured to satisfy \cref{eq:point-confidence-guarantee}. This subset includes the \emph{conditional value-at-risk}
% and the $\phi$-divergences from \cite{Duchi2021b,Lam2019}. 


% We show how the large class 
% of \emph{law-invariant, coherent risk measures} -- which are dual to DRO -- serve as high-confidence bound of the expectation.
% This suggest a large class of proxy costs satisfying \cref{eq:point-confidence-guarantee}, the value of $\varepsilon$ of which can be computed 
% tightly for every $n$, contrasting other work which only supports sufficiently large values of $n$. 
% For a subset of these law-invariant, coherent risk measures we conversely illustrate how given some $\varepsilon$ 
% the risk measure can be configured to satisfy \cref{eq:point-confidence-guarantee}. This subset includes the well known \emph{conditional value-at-risk}
% and the $\phi$-divergences considered in \cite{Duchi2021b,Lam2019}. 

% Problems like \cref{eq:expected-risk-minimization} are omnipresent in machine-learning and statistics in general \cite{Shalev-Shwartz2013,Vapnik1998}. 
% The loss function $\ell \colon \Theta \times \Xi \to \Re$ can model some estimation error 
% in the case of regression or classification \cite[\S9]{Shalev-Shwartz2013}; it can model the 
% log-likelihood of the data in the case of density estimation \cite[\S1.6]{Vapnik1998}; the return on an investment in case of 
% portfolio optimization \cite[\S1.4]{Shapiro2021}; the profit given some uncertain demand in the case of multi-product assembly \cite[\S1.3]{Shapiro2021}
% or it can model some (relaxed) chance constraint in stochastic optimal control problems \cite{Lorenzen2017}.

% In practice the expectation in \cref{eq:expected-risk-minimization} cannot be evaluated explicitly. Instead 
% a sample $\{\xi_i\}_{i=1}^n$ is available. Often \cref{eq:expected-risk-minimization} is then approximated 
% using \emph{empirical risk}
% \begin{equation}\label{eq:empirical-risk-minimization}
%     \begin{alignedat}{2}
%         & \minimize_{\theta \in \Theta} &\quad& \frac{1}{n} \sum_{i=1}^{n }\ell(\theta, \xi_i).
%     \end{alignedat}        
% \end{equation}
% Under this approximation, over-fitting will often occur. This can be mitigated through regularization -- e.g. by adding a term $\lambda \cdot \nrm{\theta}_1$ with hyperparameter $\lambda$ --
% which should render the problem stable with respect to variability in the samples. Thus over-fitting is reduced at the cost of a worse fit  \cite[\S13.2]{Shalev-Shwartz2013}. 
% This fitting-stability tradeoff (or alternatively bias-complexity tradeoff \cite[\S13.4]{Shalev-Shwartz2013}) is challenging to evaluate in practice, 
% making tuning of hyper-parameters difficult. 

% As an alternative to \cref{eq:empirical-risk-minimization} \emph{distributionally robust optimization (DRO)} considers the proxy-cost 
% \begin{equation} \label{eq:coherent-risk-functional}
%         \rho[\ell(\theta, \xi)] \dfn \max_{\mu \in \mathcal{A}} \, \int_{\xi} \ell(\theta, \xi) \di \mu(\xi),
% \end{equation}
% with the so-called  \emph{ambiguity set} $\amb$ a closed, convex set of distributions selected such that $\prob[\mu_{\star} \in \mathcal{A}] \geq 1-\varepsilon$,
% with $\mu_{\star}$ the true distribution of $\xi$. Such sets can be based on moments \cite{Delage2010}, divergence from the empirical distribution \cite{Ben-Tal2013},
% Wasserstein distance \cite{Esfahani2018b} or other statistical hypothesis tests \cite{Bertsimas2018}. 
% If this distribution is within $\amb$ then clearly the maximum is larger than $\E[\ell(\theta, \xi)]$ 
% uniformly over $\theta$. Hence 
% \begin{equation} \label{eq:uniform-confidence-guarantee}
%         \prob[\rho[\ell(\theta, \xi)] \geq \E[\ell(\theta, \xi)], \forall \theta \in \Theta] \geq 1 - \varepsilon.
% \end{equation}
% As previously observed in \cite{Duchi2021b,Lam2019}, guaranteeing that $\mu_{\star} \in \mathcal{A}$ can be overly conservative.
% This is why, in practice, the ambiguity set $\amb$ is either calibrated 
% using bootstrapping \cite{Delage2010}, asymptotic versions of \cref{eq:uniform-confidence-guarantee} \cite{Bertsimas2018, Ben-Tal2013} or using cross-validation \cite{Esfahani2018b}. 
% These methods are either computationally expensive or lack guarantees for low sample counts -- the case where over-fitting is likely to occur.

% Instead it can be helpful to initially focus on a point-wise guarantee instead of the uniform one of \cref{eq:uniform-confidence-guarantee}. 
% That is 
% \begin{equation} \label{eq:point-confidence-guarantee}
%     \prob[\rho[\ell(\theta, \xi)] \geq \E[\ell(\theta, \xi)]] \geq 1 - \varepsilon, \quad \forall \theta \in \Theta.
% \end{equation}
% This is the approach of \cite{Duchi2021b,Lam2019}. 
% They start with a DRO scheme based on $\phi$-divergence balls for $\amb$, guaranteeing \cref{eq:point-confidence-guarantee} in the limit $n \to \infty$. They show that a slight 
% increase in the radius of the ball $\amb$ suffices when both sides of the event in \cref{eq:point-confidence-guarantee} are minimized over $\theta$. 
% These guarantees however only hold for sufficiently large $n$. So over-fitting can still occur.% (cf. Figure~1(b) in \cite{Duchi2021b}). 

% We take a similar approach, viewing $\ell(\theta, \xi)$ as a scalar random variable. We show how the large class 
% of \emph{law-invariant, coherent risk measures} -- which are dual to DRO -- serve as high-confidence bound of the expectation.
% This suggest a large class of proxy costs satisfying \cref{eq:point-confidence-guarantee}, the value of $\varepsilon$ of which can be computed 
% tightly for every $n$, contrasting other work which only supports sufficiently large values of $n$. 
% For a subset of these law-invariant, coherent risk measures we coversely illustrate how given some $\varepsilon$ 
% the risk measure can be configured to satisfy \cref{eq:point-confidence-guarantee}. This subset includes the well known \emph{conditional value-at-risk}
% and the $\phi$-divergences considered in \cite{Duchi2021b,Lam2019}. 



% We suggest an alternative proxy-cost to \cref{eq:empirical-risk-minimization}, motivated by finite-sample statistics, 
% that requires less tuning. Specifically we minimize
% \begin{equation} \label{eq:proxy-cost}
% \begin{alignedat}{2}
%         \varphi^{\gamma}_n(\theta) \dfn (1 - \gamma) \CVAR^{\gamma}_n[\ell(\theta, \xi)] + \gamma \bar{\ell}(\theta).
% \end{alignedat}           
% \end{equation}
% where $\CVAR^{\gamma}_n$ denotes the empirical conditional value-at-risk -- also known as average value-at-risk, expected shortfall and the super-quantile \cite{Rockafellar2014} -- defined as 
% \begin{equation} % \label{eq:conditional-value-at-risk}
%      \CVAR^{\gamma}_n[\ell(\theta, \xi)] \dfn \inf_{\tau} \left\{ \tau + \sum_{i=1}^{n} \frac{[\ell(\theta, \xi_i) - \tau]_+}{n(1-\gamma)} \right\}.
% \end{equation}
% Here $\bar{\ell} \colon \Re^{n_\theta} \to \Re$ serves as the regularization term. Ideally it should be such that $\bar{\ell}(\theta) \geq \ell(\theta, \xi)$ for almost every $\xi$. 
% The confidence level $\gamma \in \Re$ is not viewed as a regularization parameter in this scheme, but instead is tuned automatically based on the number of samples and 
% a confidence level $\epsilon$ such that,
% for fixed $\theta \in \Re^{n_{\theta}}$,
% \begin{equation} \label{eq:confidence-guarantee}
%    \prob[\varphi^{\gamma}_n(\theta) \geq \E[\ell(\theta, \xi)]] \geq 1 - \varepsilon,
% \end{equation}
% where $\varepsilon$ is a tuning parameter that can be tuned a-priori independently of the size of the sample.\todoright{sensitivity?}

% Achieving guarantees akin to \cref{eq:confidence-guarantee} is also the objective of \emph{distributionally robust optimization (DRO)}. 
% Here one considers the proxy-cost 
% \begin{equation*}
%         \bar{\varphi}_n^{\varepsilon}(\theta) \dfn \max_{\mu \in \mathcal{A}} \, \int_{\xi} \ell(\theta, \xi) \di \mu(\xi),
% \end{equation*}
% with the so-called \emph{ambiguity set} $\amb$ of distributions selected such that $\prob[\mu_{\star} \in \mathcal{A}] \geq 1-\varepsilon$,
% with $\mu_{\star}$ the true distribution of $\xi$. Such sets can be based on moments \cite{Delage2010}, divergence from the empirical distribution \cite{Ben-Tal2013},
% Wasserstein distance \cite{Esfahani2018b} or other statistical hypothesis tests \cite{Bertsimas2018}. 
% If this distribution is within $\amb$ then clearly the maximum is larger than $\E[\ell(\theta, \xi)]$ 
% uniformly over $\theta$. Hence 
% \begin{equation} \label{eq:uniform-confidence-guarantee}
%         \prob[\bar{\varphi}^{\varepsilon}_n(\theta) \geq \E[\ell(\theta, \xi)], \forall \theta \in \Theta] \geq 1 - \varepsilon.
% \end{equation}
% This guarantee is somewhat stronger than \cref{eq:confidence-guarantee}, since the first holds uniformly over $\theta$ 
% while the second only holds pointwise. Nonetheless we observe that our method generalizes well, without any of the 
% conservativeness rampant in DRO. This is why, in practice, the ambiguity set $\amb$ is either calibrated 
% using bootstrapping \cite{Delage2010}, asymptotic versions of \cref{eq:uniform-confidence-guarantee} \cite{Bertsimas2018, Ben-Tal2013} or using cross-validation \cite{Esfahani2018b}. 
% These methods are either computationally expensive or lack guarantees for low sample counts -- the case where over-fitting is likely to occur. 

% This limitation of DRO is caused by the requirement that $\mu_{\star} \in \amb$. This is much stronger than requiring $\bar{\varphi}_{n}^{\epsilon}$
% upper bounds the expected risk. Hence other authors have started investigating this second problem directly, viewing $\ell(\theta, \xi)$ 
% as a scalar random variable, the mean of which should be bounded. In the asymptotic setting (i.e. for large $n$) progress has been made by \cite{Duchi2021b,Lam2019}. 
% They start with a DRO scheme based on $f$-divergence balls for $\amb$, guaranteeing \cref{eq:confidence-guarantee} in the limit $n \to \infty$. They then show that a slight 
% increase in the radius of the ball $\amb$ is sufficient to make the guarantee hold when both sides of \cref{eq:confidence-guarantee} are minimized over $\theta$. The fact 
% that these guarantees only hold for sufficiently large $n$ however means that over-fitting still occurs (cf. Figure~1(b) in \cite{Duchi2021b}). 

% In this work we similarly view $\ell(\theta, \xi)$ as a scalar random variable and compute a bound for the (scalar) mean, which
% holds for all $n$. The bound was first conceived by Anderson \cite{Anderson1969} and corresponds to 
% \cref{eq:proxy-cost}. The relation to $\CVAR$ is novel to the authors knowledge. 

% Unlike \cite{Duchi2021b,Lam2019}, investigation of the gap between \cref{eq:confidence-guarantee} and \cref{eq:uniform-confidence-guarantee}
% is left to future work. We instead provide a number of experimental results to illustrate that \cref{eq:confidence-guarantee} is often 
% sufficient for good generalization.

The rest of the paper proceeds as follows. In \cref{sec:statistical-framework} we derive mean bounds linked to law-invariant coherent risk measures through the distortion representation in \cref{sec:distortion-representation}. 
The problem of calibrating 
risk measures given $\varepsilon$ is answered in \cref{sec:calibration} and in \cref{sec:case-studies} numerical case 
studies are presented, showing the performance of these calibrated risks.

\ilpub{Throughout this paper we highlight the main results and provide only high-level proofs. 
A more exhaustive treatise is contained in a technical report \cite{TR}.}

\paragraph*{Notation} Let $\Re$ denote the reals\ilarxiv{\,and $\eRe$ the extended reals}. 
For some convex function $\phi \colon \Re^n \to \ilarxiv{\eRe}\ilpub{\Re}$ let $\phi^*$ denote the convex conjugate\ilarxiv{, $\partial \phi$ the subgradient} and
$\dom \phi$ its domain. 
\ilarxiv{For a set $\set{X}$ let $\iota_{\set{X}}(x) = 0$ if $x \in \set{X}$ and $+\infty$ otherwise be the indicator function of $\set{X}$ and $\ri \set{X}$ the relative interior.}
For integers $a, b$ let $[a, b] = \{a, \dots, b\}$ and $[b] = \{1, \dots, b\}$. Let $[x]_+ = \max(0, x)$. 
For real vectors $x, y \in \Re^n$ we use $\< x, y\>$ to denote the Euclidean inner product and $\one_n \in \Re^n$ is the vector of all ones. 
\ilarxiv{For a cone $\set{K}$ let $\set{K}^* \dfn \{y \colon \<x, y\> \geq 0, \forall x \in \set{K}\}$ denote its dual and $\set{K}^\circ \dfn -\set{K}^*$ its polar cone.}
\ilpub{For a cone $\set{K}$ let $\set{K}^\circ \dfn \{y \colon \<x, y\> \leq 0, \forall x \in \set{K}\}$ denote its polar cone.}
Let $\Pi^n$ denote the permutations of $[n]$ (i.e. all bijections $[n] \to [n]$). We write $\pi x = (x_{\pi(1)}, \dots, x_{\pi(n)})$
for $\pi \in \Pi^n$, $x \in \Re^n$ and similarly for sets $\pi \set{X} = \{\pi x \colon x \in \set{X}\}$. 
Similarly let $\Pi^n y = \{\pi y \colon \pi \in \Pi^n\}$ denote the orbit of $y$ under $\Pi^n$.
Let $\Re^n_{\uparrow} \dfn \{x \colon x_{1} \leq x_2 \leq \dots \leq x_n\}$ 
denote the monotone cone and $(\M^n)^\circ$ its polar (cf. \ilarxiv{\cref{prop:dual-monotone-cone}}\ilpub{\cite[Lem.~A.1]{TR}}). 
Let $\Delta^n \dfn \{\mu \colon \sum_{i=1}^n \mu_i = 1, \mu_i \geq 0, i \in [n]\}$ denote the probability simplex.
For a vector $x \in \Re^n$ let $x_{(1)} \leq x_{(2)} \leq \dots \leq x_{(n)}$ be the increasing permutation of the elements of $x$
with $x_{\uparrow} = (x_{(1)}, x_{(2)}, \dots, x_{(n)})$. 
\ilarxiv{For $x, y \in \Re^n$ let $x \slt y$ denote that $y$ majorizes $x$ \cite{Marshall2011}}.
For sets let $A + B \dfn \{a + b \colon a \in \set{A}, b \in \set{B}\}$
denote the Minkowski sum and for $x \in \Re^n$, $x + B = \{x\} + B$. 
For random variables $X, Y$ we write $X \deq Y$ to say $X$ is identically distributed to $Y$. Let $\esssup[X]$ 
denote the essential supremum. Let $X \deq \mathcal{U}(\ell, u)$ imply $X$ is uniformly distributed over $[\ell, u]$ and $X \deq \mathcal{N}(\mu, \Sigma)$ 
denote $X$ is normally distributed with mean $\mu$ and covariance $\Sigma$. 

==> content-old/statistics.tex <==
\section{Statistical Framework} \label{sec:statistical-framework}
In this section we find upper bounds for $\E[\ell(\theta, \xi)]$ that hold point-wise over $\theta$. These are related to classical results in order statistics. 
The bounds are presented to highlight the connection with the \emph{distortion representation} of law-invariant, coherent risk measures described in the next section. 
To simplify the notation, we focus on scalar random variables $Z \colon \Omega \to \Re$ defined on some abstract probability space $(\Omega, \F, \prob)$. 
Specifically, we fix the value of $\theta$ and take $Z = \ell(\theta, \xi)$. 
Then consider an \iid{} sample $(Z_i)_{i=1}^{n-1}  = (\ell(\theta, \xi_i))_{i=1}^{n-1}$ and some upper bound $\esssup[Z] \leq Z_{n} < +\infty$ -- one could take $Z_n = \sup_{\xi \in \Xi} \ell(\theta, \xi)$ --
with order statistic $Z_{(1)} \leq \dots \leq Z_{(n-1)} \leq \esssup[Z] \leq Z_{(n)}$.
We assume throughout that the expectation $\E[Z]$ is well defined. 

Throughout the section we assume that $Z$ is a continuous random variable for clarity of the exposition. The final theorem however holds for any random variable. 
For continuous $Z$ we have the following \cite[Thm.~8.7.4]{Wilks1964}.
\begin{proposition} \label{thm:elementary-coverage}
    Let $Z_{(1)} \leq \dots \leq Z_{(n-1)}$ be the order statistics of an \iid{} sample from a continuous random variable $Z$. 
    Moreover let $Z_{(0)} = -\infty$ and $Z_{(n)} \geq \esssup[Z]$. Then the random vector of so-called \emph{coverages}:
    \begin{equation*}
        W \dfn \left(F(Z_{(i)}) - F(Z_{(i-1)})\right)_{i=1}^{n}
    \end{equation*}
    is uniformly distributed over $\Delta^{n}$ with $F(z) = \prob[Z \leq z]$. 
\end{proposition}

We exploit this property by writing the expectation of $Z$ in terms of these 
coverages using the law of total expectation
\begin{align*}
    \E[Z] = \int_{-\infty}^{Z_{(n)}} Z \di F(Z) = \sum_{i=1}^{n} \int_{Z_{(i-1)}}^{Z_{(i)}} Z \di F(Z).
\end{align*}
The equality holds for any realization of the data. For each term
$\int_{Z_{(i-1)}}^{Z_(i)} Z \di F(Z) \leq Z_{(i)} \int_{Z_{(i-1)}}^{Z_(i)} \di F(Z) = Z_{(i)} W_i$. Hence
\begin{equation} \label{eq:known-distortion-bound}
    \E[Z] \leq \sum_{i=1}^{n} Z_{(i)} W_i = \<W, \hat{Z}_{\uparrow}\>,
\end{equation}
for any realization of the data. Computing the value of $W$ when only $Z_1, \dots, Z_n$ is known
is not possible in practice. Instead consider some set $\distort$ 
such that 
\begin{equation} \label{eq:confidence-distortion}
    \prob[W \in \distort] = 1 - \varepsilon   
\end{equation}
and take the supremum over its elements in \cref{eq:known-distortion-bound}. 

Such a confidence level is similar to that of ambiguity sets in classical data-driven DRO. There
$\prob[\mu_{\star} \in \amb] \geq 1 - \varepsilon$, which places randomness inside the data-driven $\amb$, 
while the true distribution $\mu_{\star}$ of $\xi$ in \cref{eq:expected-risk-minimization} is fixed and unknown. Instead in \cref{eq:confidence-distortion} $\distort$ is fixed and $W$ acts as the 
random variable, with known distribution by \cref{thm:elementary-coverage}. Thus calibrating $\distort$ is easier compared to calibrating $\set{A}$, which
requires conservative concentration inequalities. 

We summarize this discussion in a theorem.
\begin{theorem} \label{thm:distortion-bound}
    Given an \iid{} sample $\{Z_i\}_{i=1}^{n-1}$ from some random variable $Z$ and some $Z_{n} \geq \esssup[Z] < +\infty$,
    let $\hat{Z} = (Z_1, \dots, Z_n) \in \Re^{n}$. Consider some non-empty $\distort \subseteq \Re^n$ such that $\distort + (\M^n)^\circ = \distort$.
    Then
    \begin{equation} \label{eq:distortion-bound}
        \prob\left[ \sup_{\mu \in \distort} \<\mu, \hat{Z}_{\uparrow}\> \geq \E[Z] \right] \geq \prob[W \in \distort],
    \end{equation}
    for $W$ uniformly distributed over the simplex $\Delta^{n}$.
\end{theorem}
\begin{proof}
    Proof deferred to \ilarxiv{\cref{app:statistical-framework}}\ilpub{\cite[App.~B]{TR}}.
\end{proof}

Using the notation from the introduction, take $\hat{Z} = L(\theta)$ and reflect on the similarity of the $\sup$ to \cref{eq:robustified-erm}. 
The difference is that $L(\theta)$ is ordered, which leads to the \emph{distortion representation} of risk measures studied in the next section. 
Invariance $\distort + (\M^n)^\circ = \distort$ enables non-continuous random variables $Z$. 
Interestingly the distortion representation derived below automatically satisfies this property. 

